Satyam: Democratizing Groundtruth for Machine Vision

The democratization of machine learning (ML) has led to ML-based machine vision systems for autonomous driving, traffic monitoring, and video surveillance. However, true democratization cannot be achieved without greatly simplifying the process of collecting groundtruth for training and testing these systems. This groundtruth collection is necessary to ensure good performance under varying conditions. In this paper, we present the design and evaluation of Satyam, a first-of-its-kind system that enables a layperson to launch groundtruth collection tasks for machine vision with minimal effort. Satyam leverages a crowdtasking platform, Amazon Mechanical Turk, and automates several challenging aspects of groundtruth collection: creating and launching of custom web-UI tasks for obtaining the desired groundtruth, controlling result quality in the face of spammers and untrained workers, adapting prices to match task complexity, filtering spammers and workers with poor performance, and processing worker payments. We validate Satyam using several popular benchmark vision datasets, and demonstrate that groundtruth obtained by Satyam is comparable to that obtained from trained experts and provides matching ML performance when used for training.

==> 0_metadata.tex <==
\ifcameraready

\keywords{Autonomous Cars, ADAS, Collaborative Sensing, Extended Vision}

\newcommand{\grantack}[1]{
  \ifthenelse{\equal{#1}{CTA}}{\thanks{Research was sponsored by the Army Research Laboratory and was accomplished under Cooperative Agreement Number W911NF-09-2-0053 (the ARL Network Science CTA). The views and conclusions contained in this document are those of the authors and should not be interpreted as representing the official policies, either expressed or implied, of the Army Research Laboratory or the U.S. Government. The U.S. Government is authorized to reproduce and distribute reprints for Government purposes notwithstanding any copyright notation here on.}
    }{}
  \ifthenelse{\equal{#1}{CRA}}{\thanks{Research reported in this paper was sponsored in part by the Army Research Laboratory under Cooperative Agreement W911NF-17-2-0196. The views and conclusions contained in this document are those of the authors and should not be interpreted as representing the official policies, either expressed or implied, of the Army Research Laboratory or the U.S. Government. The U.S. Government is authorized to reproduce and distribute reprints for Government purposes notwithstanding any copyright notation here on.}}{}    
  \ifthenelse{\equal{#1}{NSFAvail}}{\thanks{This material is based upon work supported by the National Science Foundation under Grant No. 1705086.}}{}      
  \ifthenelse{\equal{#1}{CPSSyn}}{\thanks{This material is based upon work supported by the National Science Foundation under Grant No. 1330118 and from a grant from General Motors.}}{}        
  \ifthenelse{\equal{#1}{NeTSLarge}}{\thanks{This material is based upon work supported by the National Science Foundation under Grant No. 1413978.}}{}          
  \ifthenelse{\equal{#1}{NeTSSmall}}{\thanks{This material is based upon work supported by the National Science Foundation under Grant No. 1423505.}}{}
}

%%% Uncomment one or more of the following
%\grantack{CTA}
%\grantack{CRA}
%\grantack{NSFAvail}
%\grantack{CPSSyn}
%\grantack{NeTSLarge}
%\grantack{NeTSSmall}

\fi


%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> Satyam ArXiv/0_config.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% hyperref configuration
\PassOptionsToPackage{usenames,dvipsnames}{color} % color is loaded by hyperref
\hypersetup{unicode=true,
            colorlinks=true,
            linkcolor=blue,
            citecolor=blue,
            anchorcolor=blue,
            urlcolor=blue,
            breaklinks=true}
\urlstyle{same}

%% caption configuration
%\captionsetup{margin=10pt,font=small,labelfont=bf}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% other scaling, separation configuration, do not modify
\makeatletter
\def\maxwidth{\ifdim\Gin@nat@width>\linewidth\linewidth\else\Gin@nat@width\fi}
\def\maxheight{\ifdim\Gin@nat@height>\textheight\textheight\else\Gin@nat@height\fi}
\makeatother
% Scale images if necessary, so that they will not overflow the page
% margins by default, and it is still possible to overwrite the defaults
% using explicit options in \includegraphics[width, height, ...]{}
\setkeys{Gin}{width=\maxwidth,height=\maxheight,keepaspectratio}
\setlength{\emergencystretch}{3em}  % prevent overfull lines
\providecommand{\tightlist}{%
  \setlength{\itemsep}{0pt}\setlength{\parskip}{0pt}}
\setcounter{secnumdepth}{5}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% para spacing
\makeatletter
\let\origsection\section
\let\origsubsection\subsection
\let\origparagraph\paragraph

\renewcommand\section{\@ifstar{\starsection}{\nostarsection}}
\renewcommand\subsection{\@ifstar{\starsubsection}{\nostarsubsection}}

%% Change these to control spacing for section headers/paras

\newcommand\sectionprelude{\vspace{0ex}}
\newcommand\sectionpostlude{\vspace{0ex}}
\newcommand\subsectionprelude{\vspace{0ex}}
\newcommand\subsectionpostlude{\vspace{0ex}}

\newcommand\nostarsection[1]{\sectionprelude\origsection{#1}\sectionpostlude}
\newcommand\starsection[1]{\sectionprelude\origsection*{#1}\sectionpostlude}

\newcommand\nostarsubsection[1]{\subsectionprelude\origsubsection{#1}\subsectionpostlude}
\newcommand\starsubsection[1]{\subsectionprelude\origsubsection*{#1}\subsectionpostlude}

\makeatother

\newcommand\paraspace{\vspace*{0ex}}
\providecommand\parab[1]{\paraspace\noindent\textbf{#1}.}
\providecommand\parae[1]{\textbf{\textit{#1}}.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Change these to control figure/float spacing
\setlength{\textfloatsep}{2pt}
\setlength{\abovecaptionskip}{2pt}
\setlength{\belowcaptionskip}{-2pt}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Change these to control equation spacing
\apptocmd\normalsize{%
\abovedisplayskip=5pt
\abovedisplayshortskip=5pt
\belowdisplayskip=5pt
\belowdisplayshortskip=5pt
}{}{}

%%%%%%
\hypersetup{final}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> Satyam ArXiv/0_macros.tex <==
%%%%%%%%%%%%%%%%% Add paper-specific macros here
\newcommand{\sysname}{Satyam\xspace}
\newcommand{\satyam}{Satyam\xspace}

% Attempt to make hyperref and algorithmic work together better:
%\newcommand{\theHalgorithm}{\arabic{algorithm}}

%%% Latin abbrevs
\newcommand{\etc}{\textit{etc.}\xspace}
\newcommand{\ie}{\textit{i.e.,}\xspace}
\newcommand{\eg}{\textit{e.g.,}\xspace}
\newcommand{\etal}{\textit{et al.}\xspace}

%%% Sections, figures etc. Please use these for uniformity
\newcommand{\secref}[1]{\S\ref{#1}}
\newcommand{\figref}[1]{Figure~\ref{#1}}
\newcommand{\tabref}[1]{Table~\ref{#1}}
\newcommand{\algoref}[1]{Algorithm~\ref{#1}}
\newcommand{\eqnref}[1]{Equation~\ref{#1}}
\newcommand{\lineref}[1]{Line~\ref{#1}}

%%%a squished list that saves space
\newcommand{\squishlist}{
 \begin{list}{$\bullet$}
 		{ \setlength{\itemsep}{0pt}
 			\setlength{\parsep}{3pt}
 			\setlength{\topsep}{3pt}
 			\setlength{\partopsep}{0pt}
 			\setlength{\leftmargin}{1.5em}
 			\setlength{\labelwidth}{1em}
 			\setlength{\labelsep}{0.5em} } }


\newcommand{\squishend}{
  \end{list}  }


%%% Camera-ready macros
\ifcameraready
\newcommand{\cradd}[1]{\textcolor{blue}{#1}}
\newcommand{\cradd}[1]{\sout{\textcolor{red}{#1}}}
\fi




==> Satyam ArXiv/0_metadata.tex <==
\ifcameraready

\keywords{Autonomous Cars, ADAS, Collaborative Sensing, Extended Vision}

\newcommand{\grantack}[1]{
  \ifthenelse{\equal{#1}{CTA}}{\thanks{Research was sponsored by the Army Research Laboratory and was accomplished under Cooperative Agreement Number W911NF-09-2-0053 (the ARL Network Science CTA). The views and conclusions contained in this document are those of the authors and should not be interpreted as representing the official policies, either expressed or implied, of the Army Research Laboratory or the U.S. Government. The U.S. Government is authorized to reproduce and distribute reprints for Government purposes notwithstanding any copyright notation here on.}
    }{}
  \ifthenelse{\equal{#1}{CRA}}{\thanks{Research reported in this paper was sponsored in part by the Army Research Laboratory under Cooperative Agreement W911NF-17-2-0196. The views and conclusions contained in this document are those of the authors and should not be interpreted as representing the official policies, either expressed or implied, of the Army Research Laboratory or the U.S. Government. The U.S. Government is authorized to reproduce and distribute reprints for Government purposes notwithstanding any copyright notation here on.}}{}    
  \ifthenelse{\equal{#1}{NSFAvail}}{\thanks{This material is based upon work supported by the National Science Foundation under Grant No. 1705086.}}{}      
  \ifthenelse{\equal{#1}{CPSSyn}}{\thanks{This material is based upon work supported by the National Science Foundation under Grant No. 1330118 and from a grant from General Motors.}}{}        
  \ifthenelse{\equal{#1}{NeTSLarge}}{\thanks{This material is based upon work supported by the National Science Foundation under Grant No. 1413978.}}{}          
  \ifthenelse{\equal{#1}{NeTSSmall}}{\thanks{This material is based upon work supported by the National Science Foundation under Grant No. 1423505.}}{}
}

%%% Uncomment one or more of the following
%\grantack{CTA}
%\grantack{CRA}
%\grantack{NSFAvail}
%\grantack{CPSSyn}
%\grantack{NeTSLarge}
%\grantack{NeTSSmall}

\fi


%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> Satyam ArXiv/0_packages.tex <==
%%%% The rest of the packages
\usepackage{lmodern}
\usepackage{amssymb,amsmath,amsfonts}
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}

% use upquote if available, for straight quotes in verbatim environments
\IfFileExists{upquote.sty}{\usepackage{upquote}}{}

% use microtype if available
\IfFileExists{microtype.sty}{%
 \usepackage{microtype}
 \UseMicrotypeSet[protrusion]{basicmath} % disable protrusion for tt fonts
}{}

\usepackage{hyperref}
\usepackage{natbib} %% ACMart requires this, so we use it generically
\usepackage{graphicx,grffile}
% \usepackage{sysml2019}
\usepackage[accepted]{sysml2019}

%\usepackage{times} 

\usepackage{endnotes,epsfig}
\usepackage{multirow}
\usepackage{xspace}
\usepackage{tabularx}
\usepackage{ragged2e}
\usepackage{booktabs}
\usepackage{paralist}
\usepackage[american]{babel}
\usepackage[shortlabels]{enumitem}
\usepackage{courier,color,wrapfig}
\usepackage{xspace}
\usepackage{balance}
\usepackage{enumitem}
\usepackage{epstopdf}
\usepackage{multirow}
\usepackage{booktabs}
\usepackage{url}
\usepackage{amssymb}
\usepackage{pifont}
\usepackage{subfigure}
\usepackage{tikz}
\usepackage{comment}
\usepackage{mathtools}
\usepackage{ulem}
\usepackage{xkeyval}
%\usepackage[algo2e]{algorithm2e}
\usepackage{ifthen}
\usepackage{etoolbox}
\usepackage[margin=5pt,font=small,labelfont={bf,rm}]{caption}
%\usepackage{sepfootnotes}
\usepackage[compact]{titlesec}
\usepackage{bbding}
\usepackage{enumitem}

%this is for creating tables with fixed row width and text wrapped
\usepackage{array}
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
%this is for algorithms
\usepackage{amsmath}
%\usepackage{algorithm}
%\usepackage[noend]{algpseudocode}

%\makeatletter
%\def\BState{\State\hskip-\ALG@thistlm}
%\makeatother


%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> Satyam ArXiv/Intro3.tex <==
% \begin{figure*}[t]
% \centering
% \begin{minipage}{0.66\columnwidth}
%   \centering\includegraphics[width=0.7\columnwidth]{figs/MotivationAndAMTOverview/coco_1-Stewart-NS_2017-10-26-10-51-18-000.jpg}
%   %\vspace*{-0.15in}
%   \vspace{2mm}
%  \caption{Example of YOLO's output before fine-tuning (from data set $Cam1$) }
%  \vspace{-3mm}
% \label{fig:MotivationYoLoBefore}
% \end{minipage}
% \begin{minipage}{0.66\columnwidth}
%  \centering\includegraphics[width=0.7\columnwidth]{figs/MotivationAndAMTOverview/satyam_1-Stewart-NS_2017-10-26-10-51-18-000.jpg}
%   %\vspace*{-0.15in}
%   \vspace{2mm}
%  \caption{Example of YOLO's output after fine-tuning (from data set $Cam1$)}
%  \vspace{-3mm}
% \label{fig:MotivationYoLoAfter}
% \end{minipage}
%   \begin{minipage}{0.66\columnwidth}
%   \centering\includegraphics[width=0.9\columnwidth]{figs/MotivationAndAMTOverview/MotivationBeforeAfterFineTune.pdf}
%   %\vspace*{-0.15in}
%   \vspace{-1mm}
%  \caption{Improvement of performance with fine-tuned YOLO.}
%  \label{fig:MotivationYoLoPerformance}
%  \end{minipage}
% \end{figure*}


\section{Introduction}
\label{sec:intro}

The accuracy of deep neural network based machine vision systems depends on the groundtruth data used to train them. Practically deployed systems rely heavily on being trained and tested on groundtruth data from images/videos obtained from actual deployments. Often, practitioners start with a model trained on public data sets and then fine-tune the model by re-training the last few layers using groundtruth data on images/videos from the actual deployment~\cite{retrain1,retrain2} in order to improve accuracy in the field. \looseness=-1
%Testing and fine-tuning on groundtruth from the field becomes a \textit{periodic activity} to \textit{continuously adapt} to changing conditions (seasons and scenery) and to  maintain performance guarantees.

Obtaining groundtruth data, however, can present a significant barrier, as annotating images/videos often requires significant human labor and expertise. Today, practitioners use three different approaches to groundtruth collection. Large companies employ their own trained workforce to annotate groundtruth. Third parties such as \cite{spare5_website} and \cite{crowdflower} recruit, train and make available a trained workforce for annotation. Finally, \textit{crowdtasking platforms} such as Amazon Mechanical Turk (AMT~\cite{AMT}) provide rapid access to a pool of untrained \textit{workers} that can be leveraged to generate groundtruth annotations. 

While the first two approaches have the advantage of generating high quality groundtruth by using a trained workforce, they incur significant cost in recruitment and training, and are therefore often limited to well-funded companies. Consequently, employing a crowdtasking platform like AMT is often a preferred alternative for a large number of ML practitioners. Using AMT for obtaining groundtruth, however, presents several challenges that deter its widespread use. First, requesters may not always have the expertise needed to create user-friendly web user-interfaces to present to workers for annotation tasks. Second, worker quality varies widely in AMT, and results can be corrupted by spammers and bots, so requesters must curate results manually to obtain good groundtruth. Third, machine vision often requires groundtruth for hundreds or thousands of images and videos, and generate AMT Human Intelligence Tasks (HITs) manually is intractable, as is determining which workers need to be paid, or which workers to recruit.

% First, since each groundtruth annotation task is presented to the workers using a browser, \textit{requesters} (users of AMT) must create a user-friendly web user-interface (web-UI) tool designed for untrained workers and customized to each groundtruth annotation task. This often requires significant expertise and effort in terms of UI design and web development.

% Second, the quality of workers in AMT can vary widely and includes a significant fraction of careless workers, spammers, and even bots. Thus, requesters must manually inspect and curate the generated groundtruth data to ensure its quality. This manual curation quickly becomes intractable when there are several tens of thousands of images/videos. 

% Third, in AMT, each annotation task is posted in the form of Human Intelligence Task (HIT) -- typically one HIT per each image/video clip. Generating annotations for tens of thousands of images/videos then translates to posting and managing several tens of thousands of HITs. Managing these HITs can be daunting, if not insurmountable, and includes several challenges such as determining the appropriate  price to pay for the HITs while adhering to minimum hourly wage laws, identifying and disbursing payments to deserving workers (not spammers), filtering workers who do not perform specific tasks well, \etc   

% Last but not the least, there is often a significant effort involved in pre/post-processing of images and videos such as splitting longer videos into smaller, more manageable, chunks for annotation, and then re-assembling the obtained groundtruth.

\parab{Goal, Approach and Contributions}
In this paper, we ask: \textit{Is it possible to design a groundtruth collection system that is accessible to non-experts while also being both cost-effective and accurate?} To this end, we discuss the design, implementation, and evaluation of \satyam\footnote{The Satyam portal~\cite{satyamportal_website} is functional, but has not yet been released for public use.} (\secref{sec:overview}) which allows non-expert users to launch large groundtruth collection tasks in under a minute. 

\satyam users first place images/video clips at a cloud storage location. They then specify groundtruth collection declaratively using a web-portal. After a few hours to a few days (depending on the size and nature of the job), \satyam generates the groundtruth in a consumable format and notifies the user. Behind the scenes, in order to avoid the challenges of recruiting and managing trained annotators, \satyam leverages AMT workers, but automates generation of customized web-UIs, quality control and HIT management.

\begin{figure}[t]
  \centering
 \includegraphics[width=\columnwidth]{figs/MotivationAndAMTOverview/SatyamResult_lowres.pdf}
  \vspace*{-0.15in}
  \caption{Examples of \satyam Results on Detection, Segmentation, and Tracking.}
  \label{fig:satyamresults}
\end{figure}

\parae{High-level Specification} 
A key challenge in using AMT arises because the HIT is too low-level of an abstraction for large-scale groundtruth collection. \satyam elevates the abstraction for groundtruth collection by observing that machine vision tasks naturally fall into a small number of categories (\secref{sec:templates}), \eg classification (labeling objects in an image or a video), detection (identifying objects by drawing bounding boxes), segmentation (marking pixels corresponding to areas of interest) and a few others described in \secref{sec:templates}. \satyam allows users to specify their groundtruth requirements by providing customizable specification templates for each of these tasks. \looseness=-1

% We observe that groundtruth collection tasks can be broadly grouped into a handful of categories based on their UI requirements. For example, most {\it image classification} tasks require displaying an image to the worker and asking them to select one from a list of potential categories; {\it image localization} tasks ask the workers to draw a box around object of interest. In \sysname, we provide a suite of carefully designed user-customizable templates (refined through experiments on AMT), each addressing a specific class of UI-requirements.

\parae{Automated Quality Control} 
\satyam automates quality control in the face of an untrained workforce and eliminates the need for manual curation (\secref{sec:fusion}). It requests annotations from multiple workers for each  image/video clip. Based on the assumption that different workers make independent errors in the groundtruth annotation, \satyam employs novel {\it groundtruth-fusion} techniques that identify and piece together the ``correct parts'' of the annotations from each worker, while rejecting the incorrect ones and requesting additional annotations until the fused result is satisfactory. 
%Such automation is possible because there are a small number of groundtruth collection categories with well-defined semantics. 

\parae{Automated HIT Management - Pricing, Creation, Payment and Worker Filtering} 
\satyam automates posting HITs in AMT for each image/video in the specified storage location until the groundtruth for that image/video has been obtained. Instrumentation in \satyam's annotation web-UIs allow it to measure the time taken for each HIT. \satyam uses this information to adaptively adjust the price to be paid for various hits and ensures that it matches the requester's user-defined hourly wage rate.   \satyam determines whether or not a worker deserves payment by comparing their work against the final generated groundtruth and disburses payments to deserving workers. When recruiting workers, it uses past performance to filter out under-performing workers.

\parab{Implementation and Deployment} \satyam's implementation is architected using a collection of cloud functions that can be auto-scaled, that support asynchronous result handling with humans in the loop, and that can be evolved and extended easily. Using an implementation of \satyam on Azure, we evaluate (\secref{sec:eval}) various aspects of \sysname. We find that \satyam's groundtruth almost perfectly matches groundtruth from well known publicly available image/video data sets such as KITTI \cite{KITTI} which were annotated by experts or by using sophisticated equipment. Further, ML models re-trained using \satyam groundtruth perform identically with the same models re-trained with these benchmark datasets. We have used \satyam for over a year launching over 162,000 HITs on AMT to over 12,000 unique workers.

\parab{Examples of groundtruth generated by \satyam}
\figref{fig:satyamresults} show examples of the groundtruth generated by \satyam for detection, segmentation, and tracking, and how these compare with groundtruth from benchmark datasets. More examples are available in Figures~\ref{fig:DetResult},~\ref{fig:SegResult} and~\ref{fig:TrackingResult} and at~\cite{Tracking_samplesdropboxlink,Localization_samplesdropboxlink}.

% \parab{Example of \satyam in a practical deployment}
% Finally, we demonstrate the benefits of using \satyam in a practical deployment scenario for a \textit{vehicle detection} system that draws bounding boxes around vehicles in traffic surveillance video feeds from four busy intersections in two major US cities. We use \satyam to generate groundtruth for 10,000 images for each camera (approximately 600 person-hours of work) in under a day. Using YoLo~\cite{yolo} out-of-the box, pre-trained with images from the COCO dataset~\cite{coco}, results in a poor accuracy of around 60\% on all four cameras (\figref{fig:MotivationYoLoPerformance}). Re-training the final layer of YoLo using groundtruth generated by \satyam on 5,000 images (training set) from each camera, dramatically increases accuracy to nearly 80\%. \figref{fig:MotivationYoLoBefore} and~\figref{fig:MotivationYoLoAfter} show an example of YOLO output before and after the fine-tuning for one of the camera feeds. 

% We then show that the performance of DNNs trained on groundtruth obtained by \sysname and those provided by experts is almost identical. We study the various dynamics of the groundtruth collection process such as its temporal progress, the number of workers needed for consensus and its dependence on accuracy, the sensitivity of various parameters in the groundtruth-consensus and groundtruth-fusion algorithms etc. We find that using \sysname, we can collect groundtruth for several thousands of images in under a day. 

%\parab{Experiences}
%  Our experiences suggest three directions for future work needed to improve \satyam : techniques to %reduce visual complexity of tasks, .

% \parab{Summary of Contributions} In summary, this paper has the following contributions,
% \squishlist
% %\begin{enumerate}
% \item We present the design of \sysname, a system that takes a first attempt at tackling the challenging problem of groundtruth collection for machine vision tasks.
% \item We present novel {\it groundtruth-fusion} algorithms that allow \satyam to combine results from multiple workers to produce high quality groundtruth in the face of untrained workers.
% \item Through a thorough evaluation, we demonstrate that \satyam can indeed leverage untrained workers from crowdsourcing platforms to provide high quality groundtruth.
% \item We provide insightful experiences that were gained from our deployments of \sysname and provide future ideas to improve the efficiency of various components of \sysname.
% \squishend
% %\end{enumerate}

% \noindent
% {\bf Organization of the paper.} Since \sysname currently uses AMT, we start by describing the steps of using AMT to obtain groundtruth in \secref{sec:gt}. In \secref{sec:overview} we provide an overview of the various components of \sysname and how teach of them automate the various steps of groundtruth collection described in Section~\ref{xxx}. We then take a deep dive into the various algorithms used in \sysname such as the Groundtruth-consensus and groundtruth-fusion algorithms in \secref{sec:fusion}. We then describe the implementation and deployment of \sysname in Azure in \secref{sec:impl} followed by its evaluation in \secref{sec:eval}.


\iffalse
{
\parab{\satyam in the field - an example}
To demonstrate how \satyam can help in practical deployments  we consider a \textit{vehicle detection} system that draws bounding boxes around vehicles in traffic surveillance video feeds from four busy intersections in two major US cities. We use a popular deep-neural network, YOLO~\cite{yolo}, that comes pre-trained using images from the COCO dataset~\cite{coco} -- the YOLO-COCO model. To test its performance, we collect 10,000 HD quality images from each camera, over one week, 7:00 A.M - 7:00 P.M. \figref{fig:MotivationYoLoPerformance} shows that YOLO-COCO model performs poorly on all four cameras, with an average precision of under 60\%. This poor performance occurs because the characteristics of the specific camera footages (\eg viewing angle and background scenery) are different from those in the COCO dataset. Next, for each camera, we generate a fine-tuned model by training only the final layer of YOLO-COCO using a separate training set of 10,000 HD images from the camera. After fine-tuning, (YOLO-FineTuned), there is a dramatic improvement in accuracy, nearly 80\% for each camera. \figref{fig:MotivationYoLoBefore} and~\figref{fig:MotivationYoLoAfter} show an example of YOLO output before and after the fine-tuning. 

\parab{The challenges of obtaining groundtruth data}
The accuracy improvement, however, comes at a significant cost in human labor required to generate the training data sets from each camera. In the above example, each traffic surveillance images had between  15-25 cars per frame. A trained personnel takes on average 5~s to annotate (draw a box around) a single car, or about 140 person-hours \textit{per camera}. Practical surveillance deployments have hundreds of cameras and obtaining groundtruth requires immense manual effort. 
}\fi

==> Satyam ArXiv/abstract1.tex <==
\begin{abstract}
The democratization of machine learning (ML) has led to ML-based machine vision systems for autonomous driving, traffic monitoring, and video surveillance. However, true democratization cannot be achieved without greatly simplifying the process of collecting groundtruth for training and testing these systems. This groundtruth collection is necessary to ensure good performance under varying conditions.
% Obtaining groundtruth data for testing and training these systems, in order to provide continued performance guarantees under changing conditions, however, often presents a significant barrier for the true democratization of ML systems.
In this paper, we present the design and evaluation of \textbf{\satyam}, a first-of-its-kind system that enables a layperson to launch groundtruth collection tasks for machine vision with minimal effort. \satyam leverages a crowdtasking platform, Amazon Mechanical Turk, and automates several challenging aspects of  groundtruth collection: creating and launching of custom web-UI tasks for obtaining the desired groundtruth, controlling result quality in the face of spammers and untrained workers, adapting prices to match task complexity, filtering spammers and workers with poor performance, and processing worker payments. We validate  \satyam using several popular benchmark vision data sets, and demonstrate that groundtruth obtained by \satyam is comparable to that obtained from trained experts and provides matching ML performance when used for training. \looseness=-1
\end{abstract}

==> Satyam ArXiv/appendices.tex <==
\newpage
\appendix
\renewcommand\thefigure{A.\arabic{figure}}
\setcounter{figure}{0}

%% Datasets
%% Sensitivity
%% Portal
%% Samples
%% Examples
%% Error Analysis

\section{Appendix}
%\section{Illustrations}

% Things that should go in here:
% \begin{itemize}[topsep=1pt,itemsep=0pt,leftmargin=*]
%     \item Pseudo code for tricky algorithms
%     \item Screen shots of templates
%     \item Screen shot of worker view
%     \item Sample images for some of the tasks (tracking, localization \etc)
%     \item project webpage of aggregated results, yolo coco and satyam retrain comparison...
%     \item $\ldots$
% \end{itemize}

\begin{figure*}[t]
\centering
  \begin{minipage}{0.66\columnwidth}
  \centering
  \includegraphics[width=0.95\columnwidth]{figs/MotivationAndAMTOverview/DetectionResult_lowres.pdf}
  %\vspace*{-0.15in}
  \caption{Example Results of \satyam Detection from KITTI}
  \label{fig:DetResult}
 \end{minipage}
\begin{minipage}{0.66\columnwidth}
  \centering \includegraphics[width=0.95\columnwidth]{figs/MotivationAndAMTOverview/SegResult_lowres.pdf}
  %\vspace*{-0.15in}
  \caption{Example Results of \satyam Segmentation from PASCAL}
  \label{fig:SegResult}
\end{minipage}
\begin{minipage}{0.66\columnwidth}
 \centering\includegraphics[width=0.95\columnwidth]{figs/MotivationAndAMTOverview/TrackingResult_lowres.pdf}
  %\vspace*{-0.15in}
  \caption{Example Results of \satyam Tracking from KITTI}
  \label{fig:TrackingResult}
\end{minipage}
\end{figure*}

\subsection{ML Benchmark Datasets Used in Evaluation}
\label{sec:eval:datasets}
 
\parab{Image Classification (ImageNet-10)} We create this dataset by picking all the images corresponding to 10 classes commonly seen in video surveillance cameras from the ImageNet~\cite{ImageNet} dataset. Our dataset contains 12,482 images covering these classes: cat, dog, bicycle, lorry-truck, motorcycle, SUV, van, female person and male person.  

\parab{Video Classification (JHMDB-10)} For this data set we pick all the video clips from the JHMDB~\cite{JHMDB} data set corresponding to to 10 common human activities: clap, jump, pick, push, run, sit, stand, throw, walk and, wave (a total of 411 video clips).

\parab{Counting in Images (CAPRK-1)} We create this data set by selecting 164 drone images taken from one parking lot from CAPRK~\cite{carpk} (a total of 3,616 cars).

\parab{Object Detection in Images (KITTI-Object)}
We create this data set by considering 3 out of 8 classes (cars, pedestrians and cyclists) in the KITTI~\cite{KITTI}  data set with 8000 images (a total of 20,174 objects.). The groundtruth in KITTI established using LiDAR mounted on the car. 

\parab{Object Segmentation in Images (PASCAL-VOC-Seg)} %PASCAL-VOC \cite{pascalvoc} is a standardized image dataset for object classification, detection, segmentation, action classification, and person layout. 
We create this data set by choosing XXX images from the PASCAL-VOC \cite{pascalvoc} data set that have segmentation labels, including the groundtruth of both class- and instance-level segmentation, corresponding to a total of XXX objects of 20 different classes.

\parab{Tracking in Videos (KITTI-Trac)} For this dataset we chose all 21 video clips that were collected from a moving car from KITTI~\cite{KITTI} (about 8000 frames), but evaluate tracks only for 2 classes -- cars and pedestrians. During the pre-processing step, these 21 video clips were broken into 276 chunks of length 3 seconds each with a 0.5 second overlap between consecutive chunks.

\parab{Traffic Surveillance Video Stream Data (SURV)} We extracted images at 1~frame/minute from the video streams of 4 live HD quality traffic surveillance cameras, over one week (7 days) between 7:00~am and 7:00~pm each day. These cameras are located at major intersections in two U.S cities. We label the dataset corresponding to each of the four cameras as SURV-1, SURV-2, SURV-3 and SURV-4 respectively. 



\subsection{Samples of Groudtruth Images/Video Obtained by \satyam}
\label{sec:samples}
Figures~\ref{fig:DetResult},~\ref{fig:SegResult} and~\ref{fig:TrackingResult} show some examples of groundtruth obtained using \satyam for detection, segmentation and tracking templates respectively.



\subsection{Examples of \satyam tasks seen by workers}
\label{sec:portal}
The \satyam portal can be visited at ~\cite{satyamportal_website}. Here we provide a few example screenshots of the task pages that AMT workers see for each template in Figures~\ref{fig:imClassfication_taskpage},~\ref{fig:counting_taskpage},~\ref{fig:imDetection_taskpage},~\ref{fig:imSegmentation_taskpage}, and ~\ref{fig:tracking_taskpage}. Figure~\ref{fig:mturk} depicts a typical view of an AMT worker, when they choose among the many HITs available to them.



\begin{figure}[h]
  \centering
  \includegraphics[width=\columnwidth]{figs/appendix/ImageClassification.PNG}
  %\vspace*{-0.15in}
  \caption{Image Classification Task Page}
  \label{fig:imClassfication_taskpage}
\end{figure} 

\begin{figure}[h]
  \centering
  \includegraphics[width=\columnwidth]{figs/appendix/Counting.PNG}
  %\vspace*{-0.15in}
  \caption{Object Counting Task Page}
  \label{fig:counting_taskpage}
\end{figure}

\begin{figure}[h]
  \centering
  \includegraphics[width=\columnwidth]{figs/appendix/ImageDetection.PNG}
  %\vspace*{-0.15in}
  \caption{Object Detection and Localization Task Page}
  \label{fig:imDetection_taskpage}
\end{figure}

\begin{figure}[h]
  \centering
  \includegraphics[width=\columnwidth]{figs/appendix/Segmentation.PNG}
  %\vspace*{-0.15in}
  \caption{Object Segmentation Task Page}
  \label{fig:imSegmentation_taskpage}
\end{figure}

\begin{figure}
  \centering
  \includegraphics[width=\columnwidth]{figs/appendix/Tracking.pdf}
  %\vspace*{-0.15in}
  \caption{Multi-Object Tracking Task Page}
  \label{fig:tracking_taskpage}
\end{figure}

\begin{figure}[h]
  \centering
  \includegraphics[width=\columnwidth]{figs/appendix/mturk.PNG}
  %\vspace*{-0.15in}
  \caption{Amazon MTurk HITs Web Portal}
  \label{fig:mturk}
\end{figure} 

\subsection{Examples of Mismatches between \satyam and Benchmarks}
\label{sec:mismatches}

In this section we provide some interesting examples of mismatch between groundtruth in the benchmark data sets and that obtained by \satyam to provide insights to the reader. 

Figure~\ref{fig:vantruck1} shows errors in the classification template due to linguistic confusion where, while in ImageNet these vehicles were labeled as vans, \satyam yielded the class label as trucks.
Figure~\ref{fig:segmentation_error} shows an error by the human annotator in the benchmark dataset for the segmentation template where the human misses marking the  truck in the scene whereas these are marked in the groundtruth obtained from \satyam.
Figure~\ref{fig:count_error} is an example of the confusion that human annotators experience when counting in groundtruth data sets where there are partially visible cars which are open to interpretation of the annotator as to whether it should be included in the count.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.45\columnwidth]{figs/appendix/van_truck1.jpg}
    \includegraphics[width=0.45\columnwidth]{figs/appendix/van_truck2.jpg}
    \caption{Linguistic confusion between van and truck}
    \label{fig:vantruck1}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.32\columnwidth]{figs/appendix/2007_000364.jpg}
    \includegraphics[width=0.32\columnwidth]{figs/appendix/2007_000364.png}
    \includegraphics[width=0.32\columnwidth]{figs/appendix/2007_000364_aggregated.PNG}
    \caption{Example of missing segmentation labels from PASCAL. From left to right: raw image, PASCAL label, \satyam label. \satyam segments a small truck on the top left corner which was not present in the ground truth.}
    \label{fig:segmentation_error}
\end{figure}


% \begin{figure}[h]
%     \centering
%     \includegraphics{figs/appendix/van_truck2.jpg}
%     \caption{Another example of linguistic confusion between van and truck}
%     \label{fig:vantruck2}
% \end{figure}


\subsection{Tracking Error Analysis}
\label{sec:error}

To understand tracking errors, we explored worker performance at different positions in the chunk (\figref{fig:tracking_error_chunk}): we found that, as workers get to the end of a chunk, they tend not to start tracking new objects. Decreasing the chunk size and increasing the overlap among consecutive chunks would increase accuracy, at higher cost. 

% We have left an understanding of this to future work, in part because \satyam's groundtruth is of high-enough quality that models re-trained with \satyam perform identically with benchmark-retrained models, as we discuss next.

% A detailed analysis of errors in the tracking template indicated that a large part of the this loss in accuracy comes from the fact that workers tend to not start new tracks towards the end of the video chunk. Consequently, we believe that decreasing the chunk size and increasing the overlap among consecutive chunks will increase the accuracy, however, this comes at a higher cost, as the more workers are needed to annotate the larger number of video chunks. 

\begin{figure}
    \centering
     \includegraphics[width=\columnwidth]{figs/eval/video_confusionMat.pdf}
%   %\vspace*{-0.15in}
 \caption{Confusion Matrix of \satyam Result on JHMDB}
 \label{fig:confMatVideo}
\end{figure}


\begin{figure}[h]
    \centering
    \includegraphics[width=\columnwidth]{figs/appendix/count_error.pdf}
    \caption{Example of counting error resulting from partially visible cars}
    \label{fig:count_error}
\end{figure}

\begin{figure}
  \centering
  \includegraphics[width=\columnwidth]{figs/eval/TrackingErrorDistribution.eps}
  %\vspace*{-0.15in}
  \caption{Tracking Error Distribution over 30 Frame Video Chunk}
  \label{fig:tracking_error_chunk}
\end{figure}

\subsection{Parameter Sensitivity}
\label{sec:evaluation:paramChoices}

\satyam's groundtruth fusion and result evaluation algorithms have several parameters and \figref{fig:accuracy} presents results for the best parameter choice. We have analyzed the entire space of parameters to determine the parameters that \satyam performance most crucially depends upon in terms of accuracy, latency and cost.

Image classification is sensitive only to two parameters: $n_{min}$, the minimum number of results before aggregation can commence, and $\beta$, the fraction determining the super-majority. The upper graph in \figref{fig:param:image_classification} shows how classification accuracy varies as a function of these two parameters. Because the cost and latency of groundtruth collection varies with parameters, the lower graph shows the cost (blue bars) and the latency (red bars) for each parameter choice. From this, we can see that when $n_{min}\ge 3$  and $\beta \ge 0.7$ the accuracy does not improve significantly, however, cost and latency increase. This indicates that $n_{min}=3$ and $\beta = 0.7$ are good parameter choices, with high accuracy, while having moderate cost and latency. \looseness=-1

We have conducted similar analyses for video classification (\figref{fig:param:video_classification}), counting (\figref{fig:param:counting}), object detection (\figref{fig:param:localization}), and tracking (\figref{fig:param:tracking}). Space constraints preclude a detailed discussion, but the key conclusions are:
(a) All job categories are sensitive to $n_{min}$, the minimum number of results before \satyam attempts to aggregate results;
(b) Each category is sensitive to one other parameter. For classification, this is the $\beta$ parameter that determines the super-majority criterion. For counting, it is the error tolerance $\epsilon$. For detection and tracking, it is $\eta_{cov}$, the fraction of corroborated groundtruth elements; and
(c) In each case, there exists a parameter settings at which provides good groundtruth performance at moderate cost and latency.

\begin{figure}
  \centering
%   \includegraphics[width=2.8in]{figs/eval/ParamSweep_ImageClassification.eps}
  \includegraphics[width=0.95\columnwidth]{figs/eval/ParamSweep_ImageClassification_LargerFont.eps}
  %\vspace*{-0.15in}
  \caption{Accuracy, Latency and Cost: Image Classification}
  \label{fig:param:image_classification}
\end{figure}

\begin{figure}
  \centering
  \includegraphics[width=\columnwidth]{figs/eval/ParamSweep_VideoClassification.eps}
  %\vspace*{-0.15in}
  \caption{Accuracy, Latency and Cost: Video Classification}
  \label{fig:param:video_classification}
\end{figure}

\begin{figure}
  \centering
  \includegraphics[width=\columnwidth]{figs/eval/ParamSweep_Counting.eps}
  %\vspace*{-0.15in}
  \caption{Accuracy, Latency and Cost: Counting}
  \label{fig:param:counting}
\end{figure}

\begin{figure}
  \centering
  \includegraphics[width=\columnwidth]{figs/eval/ParamSweep_Detection.eps}
  %\vspace*{-0.15in}
  \caption{Accuracy, Latency and Cost: Detection}
  \label{fig:param:localization}
\end{figure}

\begin{figure}
  \centering
  \includegraphics[width=\columnwidth]{figs/eval/ParamSweep_Tracking.eps}
  %\vspace*{-0.15in}
  \caption{Accuracy, Latency and Cost: Tracking}
  \label{fig:param:tracking}
\end{figure}



%  \begin{figure}
%   \centering
%      \includegraphics[width=\columnwidth]{figs/eval/ApprovalTimeSeries.eps}
%   %\vspace*{-0.15in}
%   \caption{Tracking Approval rates through Worker Filtering}
%   \label{fig:trackingApprovalRate}
%  \end{figure}

% \begin{figure}
%   \centering
%   \includegraphics[width=\columnwidth]{figs/eval/ApprovalTimeSeries.eps}
%   %\vspace*{-0.15in}
%   \caption{Approval Rates of Tracking Task}
%   \label{fig:trackingApprovalRate}
% \end{figure}


==> Satyam ArXiv/conclusions.tex <==
\section{Conclusions}
\label{sec:concl}

In this paper, we have presented \satyam, a cloud-based platform for automating large-scale groundtruth collection for machine vision applications. \satyam's groundtruth matches that of existing ML benchmarks datasets, ML models retrained with \satyam are as good as those re-trained with benchmark datasets, and ML models fine-tuned with \satyam's groundtruth improve detection accuracy by up to 28\% in real deployments over pre-trained models. 
% We intend to add support for image segmentation, worker filtering, adaptive pricing, and visual complexity management techniques to \satyam in the near future. \looseness=-1
%  \satyam also includes support for worker filtering and adaptive pricing to improve the quality of the results while meeting minimum wage requirement.

==> Satyam ArXiv/emulations.tex <==



\section{Lessons and Future Work}
\label{sec:learnings}

We have had significant experience with \satyam, having launched over 162,000 HITs and 470,000 \satyam-tasks to nearly 10,000 workers in the past year or so. We now we describe lessons learned from our use of \satyam, and discuss ways to improve \satyam's efficiency and usability.

\iffalse
{
\begin{table}[h]
\centering
\footnotesize
\begin{tabular}{|l|l|l|}\hline
{\bf Web-UI Template} & {\bf Original} & {After Filtering} \\ \hline\hline
Image Classification & 89\% & 90.3\% \\ \hline
Video Classification & 88.7\% & 91.4\% \\ \hline
Localization in Images & 75\% & 82.9\% \\ \hline
Tracking in Videos & 68.1\% & 86.6\% \\ \hline
Counting in Images & 92.4\% & 94\% \\ \hline
\end{tabular}
\caption{Approval Rates for various \sysname templates}
\label{tab:approvals}
%\vspace{-0.1in}
\end{table}
}\fi
% \begin{figure}
%   \centering
%   \includegraphics[width=\columnwidth]{figs/eval/ApprovalCanary.eps}
%   %\vspace*{-0.15in}
%   \caption{Approval Rates with Worker Filtering}
%   \label{fig:workerFilter}
% \end{figure}

% \begin{figure}
%   \centering
%   \includegraphics[width=\columnwidth]{figs/eval/ApprovalTimeSeries.eps}
%   %\vspace*{-0.15in}
%   \caption{Approval Rates of Tracking Task}
%   \label{fig:trackingApprovalRate}
% \end{figure}

% \subsection{Worker Filtering}
% \label{sec:learnings:workerFiltering}


% As seen from Table~\ref{tab:approvals}, while the classification tasks have a high approval rate of over 90\%, localization and tracking tasks have a lower approval rates of 70\% and 60\% respectively. This indicates for more complex tasks, fewer fraction of untrained workers in the AMT system, perform satisfactorily. High worker rejection rates for complex tasks not only adversely effects \sysname by wasting computing resources but also wastes workers' moral as they feel they wasted their precious time. Thus, it is useful to be able to preferentially provide HITs corresponding to a job to workers who have historically performed well on that job. In order to test our hypothesis, we designed and emulated a worker filtering mechanism on data obtained from our evaluation of \sysname.

% allowing 80\% of HITs are preferentially provided to good workers while 20\% of the HITs are provided to new workers for whic
% Our mechanism must preferentially provide HITs to historically well performing workers while also exploring new workers for potential new performers. For each job, we maintain and update the approval rate for each worker as the results for the job are aggregated. Workers with approval rates higher than 50\% are deemed ``good workers'' and 80\% of the HITs are preferentially provided to these  good workers while 20\% of the HITs are provided to new workers who have not been evaluated. 

\parae{Evaluation} Table~\ref{tab:approvals} shows this simple mechanism significantly improves the approval rate of the workers for the complex templates: object detection and tracking approval rates increase by 7\% and 22\% respectively. Moreover, this mechanism works well throughout the duration of the job: with worker filtering, approval rates start high and remain higher than without approval (\figref{fig:trackingApprovalRate}).

% such as tracking from 60\% to 20\%. Figure~\ref{fig:xxx} shows how the approval rate for a tracking template job changes over time with and without filtering. As seen from Figure~\ref{fig:xxx}, worker filtering keeps the approvals consistently at a high rate and thus engaging workers who perform well. We hope to improve upon these initial algorithms for worker filtering and incorporating it into the \sysname system.

% \subsection{Adaptive Pricing}
% \label{sec:learnings:adaptivePricing}

\parab{Adaptive Pricing}
A key question often that is hard to answer for \sysname users is what should be the price of a HIT? This question is governed by two factors. First, AMT is an open market and workers like to choose HITs that pay them the most in the shortest amount of time and those that are interest them. Thus, a HIT with a price too low will remain undone. Second, while a \sysname user might want to pay as low as possible, ethics and minimum pay standards employed by companies impose constraints on the minimum hourly rates that must be paid to workers. 

%As prior work has pointed out, there is clearly a correlation between time to complete a HIT and price~\cite{xxx}.
Unfortunately, the time to complete a job depends on at least two factors. First, it depends on the job category (\figref{fig:timeCDF}): task completion times are high for more visually complex tasks like counting, detection and classification, and they also vary a lot. Within the same job category, time to complete tasks can depend on the data (\figref{fig:timeCDF_counting}): KITTI has around 10 vehicles on average, and CARPK around 45 in each image, and the distribution of worker task completion times varies significantly across these datasets. (As an aside, both these figures have a long tail: we have seen several cases where workers start tasks but sometimes finish it hours later).

Given this, we believe \satyam should support \textit{adaptive pricing}: users can specify a price range within which \satyam can adaptively adjust prices based on worker task completion rates. Such a strategy would adapt both to task complexity and visual complexity in the data. \looseness=-1

% \sysname already maintains statistics regarding how long workers take for each HIT, recording the time difference between the time the worker was served the HIT to the time it was submitted. Figure~\ref{fig:timeCDF} depicts the CDF of times taken to perform a task for each of the five templates. Task completion times depend on the complexity of the task and exhibit large variability (the x-axis is in log-scale). One strategy is to use the median value of task completion times for each job and use that for determining the price per HIT. For example, it can be used to ensure the minimum payrate constraints for each job. Further, adaptive exploration schemes can be developed that try various price points.


% \begin{figure}
%   \centering
%   \includegraphics[width=\columnwidth]{figs/eval/timePerResult.eps}
%   %\vspace*{-0.15in}
%   \caption{CDF of Time Spent Per Task of All Job Categories}
%   \label{fig:timeCDF}
% \end{figure}

% \begin{figure}
%   \centering
%   \includegraphics[width=\columnwidth]{figs/eval/countingTimePerResult.eps}
%   %\vspace*{-0.15in}
%   \caption{CDF of Time Per Counting Task over Different Datasets}
%   \label{fig:timeCDF_counting}
% \end{figure}

% \subsection{Managing Cognitive Complexity}
% \label{sec:learning:cognitivecomplexity}

\parab{Managing Cognitive Complexity}
Although we have tested \satyam on images with significant visual complexity (\eg 20-30 cars) and workers seem to perform well, \satyam will need mechanisms to adapt to visual complexity to avoid cognitive overload. It already uses a simple, non-adaptive strategy: chunking video clips into fixed length segments to manage cognitive overload. We arrived at this strategy by experimenting with longer videos and finding that no worker completed these tasks. \satyam could adaptively determine, based on HIT uptake, whether a particular job has high cognitive load, then, adapt chunk sizes dynamically for video, or tesselate images. \looseness=-1

\parab{A Unifying Mechanism: The Canary}
The adaptive capabilities described above require estimates for worker approval rates and task completion times. These depend not just on the job category, but also on the complexity of the data itself. We are currently experimenting with a \textit{canarying} mechanism, whereby \satyam sends a small fraction of the user-submitted data to workers to learn these parameters, then uses these when obtaining groundtruth for the complete set.





==> Satyam ArXiv/evaluation.tex <==
% \begin{figure*}[h]
%   \centering
%   \begin{minipage}{2.9in}
%   \centering
%   \includegraphics[width=2.9in]{figs/eval/Accuracy.png}
%   %\vspace*{-0.15in}
%   \caption{\satyam Accuracy, Latency, and Cost}
%   \label{fig:accuracy}
%   \end{minipage}
%   \begin{minipage}{2.0in}
%   \centering
%   \includegraphics[width=2.0in]{figs/eval/image_confusionMat_Percentage.eps}
%   %\vspace*{-0.15in}
%  \caption{Confusion Matrix of \satyam Result on ImageNet-10}
%   \label{fig:confMat}
%   \end{minipage}
%     \begin{minipage}{2.0in}
%   \centering
%   \includegraphics[width=2.0in]{figs/eval/video_confusionMat_Percentage.eps}
%   %\vspace*{-0.15in}
%  \caption{Confusion Matrix of \satyam Result on JHMDB}
%   \label{fig:confMatVideo}
%   \end{minipage}
% \end{figure*} 







% \iffalse
% {
% \begin{figure}
%   \centering
%   \includegraphics[width=\columnwidth]{figs/eval/accuracy.eps}
%   %\vspace*{-0.15in}
%   \caption{\satyam Aggregation Accuracy, Latency, and Cost}
%   \label{fig:accuracy}
% \end{figure}

% \begin{figure}
%   \centering
%   \includegraphics[width=2.0in]{figs/eval/image_confusionMat_Percentage.eps}
%   %\vspace*{-0.15in}
%  \caption{Confusion Matrix of \satyam Result on ImageNet-10}
%   \label{fig:confMat}
% \end{figure}

% \begin{figure}
%   \centering
%   \includegraphics[width=2.0in]{figs/eval/video_confusionMat_Percentage.eps}
%   %\vspace*{-0.15in}
%  \caption{Confusion Matrix of \satyam Result on JHMDB}
%   \label{fig:confMatVideo}
% \end{figure}
% }\fi

\section{Evaluation}
\label{sec:eval}

We have implemented all components (\figref{fig:Satyam-Components}) of \satyam on Azure. Our implementation is 13635 lines of C\# code. Using this, we evaluate \sysname by comparing the fidelity of its groundtruth against public \textit{ML benchmark} datasets. In these benchmarks, groundtruth was curated/generated by trained experts or by using specialized equipment in controlled settings. 
To demonstrate \sysname's effectiveness in a real world deployment we generate a data set by extracting images from four video surveillance streams at major traffic intersections in two US cities.

We evaluate \satyam along the following dimensions:
 (a) The quality of ground truth obtained by \sysname compared with that available in popular benchmark data sets;
(b) The \textit{accuracy} of deep neural networks trained using groundtruth obtained by \sysname compared with those trained using benchmark data sets;
 (c) The efficacy of fine-tuning in a deployed real-world vision-based system;
 (d) The \textit{cost} and \textit{time} to obtain groundtruth data using \sysname and; 
 (e) The efficacy of our adaptive pricing and worker filtering algorithms 
(f) The sensitivity of groundtruth-fusion algorithms to parameters.

%In order to establish the fidelity of groundtruth obtained by \sysname, we make use of popular public benchmark ML data sets whose groundtruth was curated/generated by trained experts or by using specialized equipment in controlled settings. Our approach is to independently obtain groundtruth for these data sets using \sysname and compare it with the provided benchmark groundtruth. To demonstrate, \sysname's effectiveness in a real world deployment we generate a data set by extracting images from four video surveillance streams at major traffic intersections in two US cities. 
% We start by briefly describing these data sets.


%\iffalse{
 \subsection{ML Benchmark Datasets}
 \label{sec:eval:datasets}
  
 \parab{Image Classification (ImageNet-10)} We create this dataset by picking all the images corresponding to 10 classes commonly seen in video surveillance cameras from the ImageNet~\cite{ImageNet} dataset. Our dataset contains 12,482 images covering these classes: cat, dog, bicycle, lorry-truck, motorcycle, SUV, van, female person and male person.  

 \parab{Video Classification (JHMDB-10)} For this data set we pick all the video clips from the JHMDB~\cite{JHMDB} data set corresponding to to 10 common human activities: clap, jump, pick, push, run, sit, stand, throw, walk and, wave (a total of 411 video clips).

 \parab{Counting in Images (CAPRK-1)} We create this data set by selecting 164 drone images taken from one parking lot from CAPRK~\cite{carpk} (a total of 3,616 cars).

 \parab{Object Detection in Images (KITTI-Object)}
 We create this data set by considering 3 out of 8 classes (cars, pedestrians and cyclists) in the KITTI~\cite{KITTI}  data set with 8000 images (a total of 20,174 objects.). The groundtruth in KITTI established using LiDAR mounted on the car. 

 \parab{Object Segmentation in Images (PASCAL-VOC-Seg)} PASCAL-VOC \cite{pascalvoc} is a standardized image dataset for object classification, detection, segmentation, action classification, and person layout. 
 We create this data set by choosing 353 images from the PASCAL-VOC \cite{pascalvoc} data set that have segmentation labels, including the groundtruth of both class- and instance-level segmentation, corresponding to a total of 841 objects of 20 different classes.

 \parab{Tracking in Videos (KITTI-Trac)} For this dataset we chose all 21 video clips that were collected from a moving car from KITTI~\cite{KITTI} (about 8000 frames), but evaluate tracks only for 2 classes -- cars and pedestrians. During the pre-processing step, these 21 video clips were broken into 276 chunks of length 3 seconds each with a 0.5 second overlap between consecutive chunks.

 \parab{Traffic Surveillance Video Stream Data (SURV)} We extracted images at 1~frame/minute from the video streams of 4 live HD quality traffic surveillance cameras, over one week (7 days) between 7:00~am and 7:00~pm each day. These cameras are located at major intersections in two U.S cities. We label the dataset corresponding to each of the four cameras as SURV-1, SURV-2, SURV-3 and SURV-4 respectively.    
% }\fi

% \iffalse{
% \subsection{How accurate are the Bechamark Data Sets Themselves?}
% \label{sec:eval:bechmarkAccuracy}
% The benchmark data sets, ImageNet-10, JHMB-10 and CAPRK-1 were annotated by humans and are not immune to ambiguous human interpretation. As we present  later in this section, while comparing \sysname's groundtruth we encoutered specific examples of such ambiguous categories and counts.
% Groundtruth in KiTTi-Trac and KiTTi detect was obtained not by humans by using LiDAR, which is known to be more accurate and the human eye~\cite{xxx}. Consequently, in a few cases it may not be possible even for humans to recognize a few objects. Consequently, we coin the terms {\it match-precision} and {\it match-recall} while comparing to benchmarks to indicate how closely we match the benchmark groundtruths.
% }\fi


\begin{figure*}[t]
\centering
  \begin{minipage}{0.66\columnwidth}
  \centering
  \includegraphics[width=0.95\columnwidth]{figs/MotivationAndAMTOverview/DetectionResult_lowres.pdf}
  %\vspace*{-0.15in}
  \caption{Example Results of \satyam Detection from KITTI}
  \label{fig:DetResult}
 \end{minipage}
\begin{minipage}{0.66\columnwidth}
  \centering \includegraphics[width=0.95\columnwidth]{figs/MotivationAndAMTOverview/SegResult_lowres.pdf}
  %\vspace*{-0.15in}
  \caption{Example Results of \satyam Segmentation from PASCAL}
  \label{fig:SegResult}
\end{minipage}
\begin{minipage}{0.66\columnwidth}
 \centering\includegraphics[width=0.95\columnwidth]{figs/MotivationAndAMTOverview/TrackingResult_lowres.pdf}
  %\vspace*{-0.15in}
  \caption{Example Results of \satyam Tracking from KITTI}
  \label{fig:TrackingResult}
\end{minipage}
\end{figure*}

\subsection{Quality of \sysname Groundtruth}
\label{sec:evaluation:accuracy}

%To evaluate each job category, we obtained subsets of well known public benchmarks.
%For example, ImageNet-10 was created by picking all the images corresponding to 10 classes commonly seen in video surveillance cameras from ImageNet~\cite{ImageNet}. Figure~\ref{fig:accuracy} lists the benchmark datasets, and their size, and \secref{sec:eval:datasets} describes these in detail. 

% he name of the data set used to evaluate a job category is provided in , along with a detailed description provided in Appendix~\ref{xxx}. Figure~\ref{fig:accuracy} also provides the number of annotated objects in each of the data sets.   

To demonstrate that \satyam groundtruth is comparable to that in the ML benchmarks, we launched a job in \satyam for each of the six benchmark data sets described in \figref{fig:accuracy}. Figures~\ref{fig:DetResult},~\ref{fig:SegResult} and~\ref{fig:TrackingResult} show some examples of groundtruth obtained using \satyam for detection, segmentation and tracking templates respectively. For this comparison, we evaluate \textit{match-precision} (the degree to which \satyam's groundtruth matches that of the benchmark) and \textit{match-recall} (the degree to which \satyam's workers identify groundtruth elements in the benchmark).

Figure~\ref{fig:accuracy} summarizes \sysname's accuracy for the various templates relative to the benchmarks. \satyam has uniformly high match-precision (95-99\%) and high match-recall ($>$95\%) for the relevant benchmarks. We find that \satyam often deviates from the benchmark because \textit{there are fundamental limits achieving accuracy with respect to popular benchmark data sets}, for two reasons. First, some of the benchmarks were annotated/curated by human experts and have a small fraction of errors or ambiguous annotations themselves. Some of the ambiguity, especially in classification, arises from linguistic confusion between class labels (\eg distinguishing between van and truck). Second, in others that were generated using specialized equipment (\eg LiDAR), part of the generated groundtruth is not perceivable to human eye itself. In the rest of this section, we describe our methodology for each job category and elaborate on these fundamental limits.

% In this section we wish to demonstrate that the groundtruth generated by \sysname is at par with the popular ML benchmark data sets by comparing them.
% Since \sysname's groundtruth is arrived at by combining 10 or more human workers we expect it to be at least as good a single human's performance. 
% Figure~\ref{fig:accuracy} summarizes \sysname's accuracy for the various templates assuming that the benchmark groundtruth to be correct. As seen from Figure~\ref{fig:accuracy}, while \sysname has very high accuracy, (95\%-99\%) it is still not 100\% for any of the templates. Our investigations as to the cause for this error revealed an interesting discovery -- {\it there are fundamental limits achieving accuracy with respect to popular benchmark data sets} because of two reasons. First, some of the benchmark data sets that were annotated/curated by human experts have a small fraction of errors or ambiguous annotations themselves. Second, in others data sets that were generated using specialized equipment (e.g. LiDAR), part of the generated groundtruth may not be perceivable to human eye itself. In the rest of this section we describe in detail our methodology for each template and the cause of discrepancies, albeit minor, with the benchmark data sets. 

\begin{figure}
    \centering
     \includegraphics[width=\columnwidth]{figs/eval/accuracy_final.pdf}
  %\vspace*{-0.15in}
  \caption{\satyam Accuracy, Latency, and Cost}
  \label{fig:accuracy}
\end{figure}



\parab{Image Classification}
\sysname groundtruth for ImageNet-10 has a match-precision of 98.5\% and a match-recall of 99.1\%. The confusion matrix (\figref{fig:confMat}) for all the 10 categories in ImageNet-10, shows that the largest source of mismatch is from 10\% of vans in ImageNet being classified as lorry-trucks by \satyam. We found that all of vehicles categorized as vans in ImageNet are in fact food or delivery trucks (\eg \figref{fig:vantruck1}), indicating \textit{linguistic confusion} on the part of workers. The only other significant off-diagonal entry in \figref{fig:confMat} at 1.6\% results from linguistic confusion between Vans and SUVs. Discounting these two sources of error, \satyam matches 99.9\% of the groundtruth.

\begin{figure}
    \centering
    \includegraphics[width=0.45\columnwidth]{figs/appendix/van_truck1.jpg}
    \includegraphics[width=0.45\columnwidth]{figs/appendix/van_truck2.jpg}
    \caption{Linguistic confusion between van and truck}
    \label{fig:vantruck1}
\end{figure}


\begin{figure*}
\centering
\begin{minipage}{0.66\columnwidth}
    \centering
    \includegraphics[width=0.9\columnwidth]{figs/eval/image_confusionMat_Percentage1.pdf}
  %\vspace*{-0.15in}
 \caption{Confusion Matrix of \satyam Result on ImageNet-10}
  \label{fig:confMat}
\end{minipage}
\begin{minipage}{0.66\columnwidth}
    \centering
     \includegraphics[width=\columnwidth]{figs/eval/video_confusionMat_Percentage1.eps}
%   %\vspace*{-0.15in}
 \caption{Confusion Matrix of \satyam Result on JHMDB}
 \label{fig:confMatVideo}
\end{minipage}
\begin{minipage}{0.66\columnwidth}
    \centering
    \includegraphics[width=0.95\columnwidth]{figs/appendix/count_error.pdf}
    \caption{Example of counting error resulting from partially visible cars}
    \label{fig:count_error}
\end{minipage}
\end{figure*}



\parab{Video Classification}
\satyam's groundtruth for this category set has a match-precision and match recall exceeding 99\%. The confusion matrix (\figref{fig:confMatVideo}) for the 10 categories in JHMDB-10 reveals only 3 mismatches compared to the benchmark groundtruth. We examined each case, and found that the errors resulted from class label confusion or from incorrectly labeled groundtruth in the benchmark:
a person picking up his shoes was labeled as \textit{standing} instead of \textit{picking}; a person moving fast to catch a taxi was labeled as \textit{walking} instead of \textit{running}; and finally a person who was picking up garbage bags and throwing them into a garbage truck was labeled as \textit{picking up} in JHMDB-10, while \satyam's label was \textit{throwing}. Discounting these cases, \satyam matches 100\% with the groundtruth.




\parab{Counting in Images}
\satyam's car counts deviate from the CAPRK-I benchmark's count groundtruths by 3\% (\figref{fig:accuracy}), which corresponds to an error of 1 car in a parking lot with 30 cars. This arises because of cars that are only partially visible in the image (\eg \figref{fig:count_error}), and workers were unsure whether to include these cars in the count or not. By inspecting the images we found that between 3 and 10\% of the cars in each image were partially visible. 




% The match here is computed as the ratio of the car count by \sysname in the parking lot image divided by the number of cars in the benchmark groundtruth data set CAPRK-I. As seen from Figure~\ref{fig:accuracy}, there is a 3\% mismatch in counts between \sysname's groundtruth and CAPRK's groundtruth. Further investigation revealed that this mismatch is  a result of cars that appear only partially in the image (\figref{fig:count_error}). We found that between 3-10\% of the cars in each image were only partially visible in the image frame, leading to a confusion among turk workers as to whether these cars need to be counted. Further, note that 3\% error results from a counting error of even 1 car among 30 cars in a paring lot.

\parab{Object Detection in Images}
For quantifying the accuracy for this template, we adopt the methodology recommended by the KiTTI benchmark -- two bounding boxes are said to match if their IoU is higher than a threshold. \sysname has a high match-precision of 99\% and match-recall of 97\% (\figref{fig:accuracy}). The match-recall is expected to be lower than match-precision: the LiDAR mounted on KITTI's data collection vehicle can sometimes detect objects that may not be visible to the human eye.

\parab{Object Segmentation in Images} We use Average Precision (AP)~\cite{pascalvoc} to quantify the accuracy. We use a range of IoUs (0.5-0.95 with steps of 0.05) to compute the average to avoid a bias towards a specific value. \satyam achieves an AP of 90.03\%. We also provide a match-precision of 94.77\% and a match-recall of 94.56\% using an IoU of 0.5. The dominant cause of false positives is missing annotations in the ground-truth. \figref{fig:segmentation_error} shows examples of such missing annotations from PASCAL that \satyam's users were able to produce. The primary cause of false negatives is that our experiments used a lower value of $\eta_{cov}$ than appropriate for this task; we are rectifying this currently.

\begin{figure}
    \centering
    \includegraphics[width=0.32\columnwidth]{figs/appendix/2007_000364.jpg}
    \includegraphics[width=0.32\columnwidth]{figs/appendix/2007_000364.png}
    \includegraphics[width=0.32\columnwidth]{figs/appendix/2007_000364_aggregated.PNG}
    \caption{Example of missing segmentation labels from PASCAL. From left to right: raw image, PASCAL label, \satyam label. \satyam segments a small truck on the top left corner which was not present in the ground truth.}
    \label{fig:segmentation_error}
\end{figure}

\parab{Object Tracking in Videos}
A track is a sequence of bounding boxes across multiple frames. Consequently,  we use the same match criterion for this template as detection across all the video frames. As seen from (\figref{fig:accuracy}), \sysname has a match-precision and match-recall of around 95\%. To understand why, we explored worker performance at different positions in the chunk: we found that, as workers get to the end of a chunk, they tend not to start tracking new objects. Decreasing the chunk size and increasing the overlap among consecutive chunks would increase accuracy, at higher cost. 

% (\figref{fig:tracking_error_chunk})
% , in part because \satyam's groundtruth is of high-enough quality that models re-trained with \satyam perform identically with benchmark-retrained models, as we discuss next.

% Further analysis of the errors indicated that a large part of the this loss in accuracy comes from the fact that workers tend to not start new tracks towards the end of the video chunk. Consequently, we believe that decreasing the chunk size and increasing the overlap among consecutive chunks will increase the accuracy, however, this comes at a higher cost, as the more workers are needed to annotate the larger number of video chunks.  

\begin{figure*}[t]
  \centering
  \begin{minipage}{0.66\columnwidth}
    \centering
    \includegraphics[width=0.95\columnwidth]{figs/eval/TrainingAccuracy.pdf}
  %\vspace*{-0.15in}
  \caption{Training Performance of \satyam}
  \label{fig:TrainingAccuracy}
  \end{minipage}
  \begin{minipage}{0.66\columnwidth}
    \centering
  \includegraphics[width=0.95\columnwidth]{figs/eval/TrainingAccuracy_End2End.pdf}
  %\vspace*{-0.15in}
  \caption{End to End Training using \satyam Labels}
  \label{fig:E2ETrainingAccuracy}
  \end{minipage}
 \begin{minipage}{0.66\columnwidth}
  \centering
  \includegraphics[width=0.9\columnwidth]{figs/eval/timePerResult3.pdf}
  %\vspace*{-0.15in}
  \caption{CDF of Time Spent Per Task of All Job Categories}
  \label{fig:timeCDF}
\end{minipage}
\end{figure*} 


\subsection{Re-training Models using \sysname}
\label{sec:evaluation:trainingPerformance}

A common use case for \satyam is fine-tuning ML models for improving their performance using data specific to a deployment (similar to example in Section~\ref{sec:intro}). In this section, we validate this observation by showing that (\figref{fig:TrainingAccuracy}): a) re-training ML models using \satyam groundtruth outperforms off-the-shelf pre-trained models, and b) models retrained using \satyam groundtruth perform comparably with models retrained using benchmarks. When re-training and testing a model, either with \satyam or benchmark groundtruth, we use standard methodology to train on 80\% of the data, and test on 20\%. In all cases, we retrain the last layer using accepted methodology~\cite{retrain1,retrain2}.

% In this section we demonstrate that training deep neural networks using groundtruth generated by \satyam is a) better than off-the-shelf pre-trained models, b) equivalent to that of using the groundtruth generated by experts. In order to demonstrate this, we use public datasets to fine-tune well known deep neural networks using both \satyam labels and public labels, and compare their final accuracy as well as training times with respect to each other against the off-the-shelf baseline performance, and show that they are almost the same. 

\iffalse{
\begin{figure}
  \centering
  \includegraphics[width=0.9\columnwidth]{figs/eval/TrainingAccuracy.eps}
  %\vspace*{-0.15in}
  \caption{Training Performance of \satyam}
  \label{fig:TrainingAccuracy}
\end{figure}
}\fi

\parab{Image Classification}
For this job category, we evaluate retraining a well-known state-of-the-art image classification neural network, Inception (V3) \cite{inception}. The original model was pre-trained on ImageNet-1000 \cite{ImageNet} for 1000 different classes of objects. Using this model as-is on ImageNet-10 yields a classification accuracy (F1-score~\cite{F1score}) of about 60\% (\figref{fig:TrainingAccuracy}). Retraining the models using the ImageNet-10 groundtruth increases their accuracy to 94.76\%, while retraining on \satyam results in an accuracy of 95.46\%.


% Taking the top-1 predictions of Inception on ImageNet-10, the baseline precision of Inception V3 on is merely 28.54\%. Only 4 of the 10 classes were selected and pre-trained, of which the precision is 60.43\%.  After retraining the last layer for 4000 iterations with a batch size of 100, both ImageNet original labels and Satyam labels is able to fine-tune Inception to achieve high precision (94.76\% and 95.46\%).

% \parab{Video Classification}

\parab{Object Detection in Images}
For this category, we evaluate YOLO~\cite{yolo}, pre-trained on the MS-COCO dataset. Our measure of accuracy is the mean average precision~\cite{meanAP}, a standard metric for object detection and  localization that combines precision and recall by averaging precision over all recall values. The pre-trained YOLO model has high (80\%) mean average precision, but retraining it using KITTI-Object increases this to 90.1\%. Retraining YOLO using \satyam groundtruth matches KITTI-Object's performance, with a mean average precision of 91.0\% (\figref{fig:TrainingAccuracy}).

\parab{Tracking in Videos}
% Most state-of-the-art multi-object tracking algorithms~\cite{MDP} first localize objects in each frame, then track the object across frames using a separate tracking algorithm. Recent work~\cite{goturn} has turned towards a \textit{one-shot} solution that trains a neural network to perform both tasks at once. Nevertheless, 
As of this writing, the highest ranked open-source tracker on the KITTI Tracking Benchmark leaderboard is MDP~\cite{MDP}, so we evaluate this tracker (with YOLO as the underlying object detector) using the standard Multi-Object Tracking Accuracy (MOTA~\cite{MOT_Metric}) metric, which also combines precision and recall. MDP using YOLO-CoCo's detections achieves a MOTA of 61.83\% as depicted in \figref{fig:TrainingAccuracy} but fine-tuning Yolo's last layer using the labels from KITTI and \satyam improve MOTA to  78\% and 77.77\% respectively. Further investigation reveals that the improvement in MoTA from fine-tuning was primarily due to improvement in recall -- while precision was already high (98\%) before fine-tuning, recall was only 63.54\%. After fine-tuning recall improved to 81.70\% for KITTI and 83.24\% for \sysname.

% bounding box proposal / object recognition and tracking. Well-established MOT benchmarks \cite{MOTBenchmark}\cite{KITTI} even provide detections for algorithm to use.  Nevertheless, the computer vision community has just started to look at one-shot solutions, embedding tracking into recognition models. For example, GOTURN \cite{goturn} feeds consecutive frames to a neural network which is trained to not only recognize but also track the object of interest.  

% In this experiment, we use the highest ranked open-source tracker, MDP \cite{MDP}, on KITTI Tracking Benchmark Leaderboard, and use YOLO as the detection part. In addition to precision and recall, \figref{fig:TrainingAccuracy} compares the tracking accuracy using the standard Multi-Object Tracking Accuracy (MOTA) \cite{MOT_Metric} metric. MDP using Yolo-coco's detections achieves a MOTA of 61.83\%, with 98.02\% precision, but a very low recall of 63.54\%.  Both fine-tuning yolo's last layer using the labels from KITTI and \satyam can improve MOTA (77.99\% and 77.77\%) by dramatically improving recall to 81.70\% and 83.24\%.

\begin{figure}
   \centering\includegraphics[width=0.8\columnwidth]{figs/MotivationAndAMTOverview/MotivationBeforeAfterFineTune.pdf}
  \caption{Improvement of performance with fine-tuned YOLO.}
  \label{fig:MotivationYoLoPerformance}
\end{figure}
% \parab{Counting in Images}

% The parameter $n_{min}$ -- the minimum number of workers a task is sent to is common across all the templates. For each of the templates, we 
%\subsection{Fine-Tuning ML Deployments}


\begin{figure*}
\centering
\begin{minipage}{0.66\columnwidth}
  \centering
\includegraphics[width=\columnwidth]{figs/eval/countingPDF2.pdf}
  \vspace*{-0.2in}
  \caption{Histogram of Time Per Counting Task over Different Datasets}
  \label{fig:timeCDF_counting}
\end{minipage}
\begin{minipage}{0.66\columnwidth}
  \centering
  \includegraphics[width=\columnwidth]{figs/eval/adaptivePricing.eps}
  \vspace*{-0.2in}
  \caption{Adaptive Pricing on Counting Task}
  \label{fig:adaptivePricing}
\end{minipage}
\begin{minipage}{0.66\columnwidth}
\centering
  \vspace{4mm}
  \includegraphics[width=0.95\columnwidth]{figs/eval/workerFiltering.pdf}
  \vspace{4mm}
  \caption{Approval Rates for various \sysname templates}
\label{tab:approvals}
\end{minipage}
\end{figure*}

\subsection{\sysname In Real-World Deployments}
\label{sec:evaluation:SURVData}

In order to evaluate the impact of using \satyam in the real world, we extracted images at 1~frame/minute from the video streams of 4 live HD quality traffic surveillance cameras (labeled SURV-1 to SURV-4), over one week (7 days) between 7:00~am and 7:00~pm each day. These cameras are located at major intersections in two U.S cities.
% We label the dataset corresponding to each of the four cameras as SURV-1, SURV-2, SURV-3 and SURV-4 respectively.    

We now show that using \satyam groundtruth to fine-tune ML models can result in improved classification, detection, and tracking performance. For this, we use the SURV dataset, which has surveillance camera images from four intersections, to obtain ground-truth with \satyam, then re-trained YOLO-CoCo~\cite{retrain1,retrain2} with 80\% of the ground-truth and tested on the remaining 20\%.

\satyam re-training can improve YOLO-CoCo performance uniformly across the four surveillance cameras (\figref{fig:MotivationYoLoPerformance}). The average precision improves from 52-61\% for the pre-trained models to 73-88\% for the fine-tuned models -- an improvement of 20-28\%. This validates our assertion that camera fine-tuning will be essential for practical deployments, motivating the need for a system like \satyam. 
%In preliminary experiments with these surveillance cameras, we have also found that fine-tuning models further based on lighting conditions can result in dramatic improvements: models tuned for cloudy conditions degrade significantly under bright light.

\figref{fig:E2ETrainingAccuracy} demonstrates that these benefits carry over to other job categories as well and shows fine-tuning Inception v3 for classification for one of the cameras, SURV-3. To compute this result, we used our groundtruth data from SURV-3 for the detection task, where workers also labeled objects, then trained Inception to focus on one object type, namely cars. While the pre-trained Inception model works poorly on SURV-3, fine-tuning the model results in an almost perfect classifier. Similarly, fine-tuning also results in an almost 40\% improvement in the MOTA metric for the tracker. 

% The detection result in \figref{fig:E2ETrainingAccuracy} is the same as the result for Camera 3 in \figref{fig:MotivationYoLoPerformance}.

 




\begin{figure*}
\centering
\begin{minipage}{0.66\columnwidth}
  \centering
\includegraphics[width=\columnwidth]{figs/eval/ParamSweep_ImageClassification_LargerFont.eps}
  %\vspace*{-0.15in}
  \caption{Accuracy, Latency and Cost: Image Classification}
  \label{fig:param:image_classification}
\end{minipage}
\begin{minipage}{0.66\columnwidth}
  \centering
  \includegraphics[width=\columnwidth]{figs/eval/ParamSweep_Detection.eps}
  %\vspace*{-0.15in}
  \caption{Accuracy, Latency and Cost: Detection}
  \label{fig:param:localization}
\end{minipage}
\begin{minipage}{0.66\columnwidth}
\centering
 \includegraphics[width=\columnwidth]{figs/eval/ParamSweep_Tracking.eps}
  %\vspace*{-0.15in}
  \caption{Accuracy, Latency and Cost: Tracking}
  \label{fig:param:tracking}
\end{minipage}
\end{figure*}


\subsection{Time-to-Completion and Cost}
\label{sec:evaluation:latency_cost}

\figref{fig:accuracy} also shows the median time to complete an entire job, which ranges from 7 hours to 7 days. From this, we can derive the median latency per object, which  ranges from 2.5 seconds/image for image classification to 125 seconds/object for tracking. That figure also shows the cost of annotating an object in \textit{person-seconds/object}: the actual dollar figure paid is proportional to this (\secref{sec:evaluation:priceAdaptation}). By this metric (\figref{fig:accuracy}), image and video classification, and counting cost few tens of person-seconds/object while detection,  segmentation, and tracking require 160,  599, and 978 person-seconds respectively.

% \sysname is also instrumented to collect various statistics for each job such as task completion latency, time taken to complete each task by a worker, the number of paid and unpaid tasks, \etc. In this section we try and answer the question, 
% %This data can provide estimates to help users answer two questions: a) 
% {\it how long will it take to get annotated data for a particular job?} 
% %and b) {\it how much will it cost to get the annotated data?}

% \parab{Time To Completion} The median time to completing an entire job (Median Latency [hrs], \figref{fig:accuracy}) for different job categories varies from 7 hours to 7 days depending on the volume and complexity of the tasks. Knowing the number of objects annotated in each job (\# Objects Annotated) we can compute the median latency per object annotated (Median Latency/Object in \figref{fig:accuracy}). This time is a function of several factors such as complexity of the task, number of interested active workers, \etc, and ranges from 2.5 seconds/image for image classification to 125 seconds/object for tracking. Knowing the size and characteristics of their dataset, and using these estimates, \satyam can approximately determine how long the jobs are likely to take.

% \parab{Time (Cost) to Annotating an Object}
% A good measure of the cost of annotation is person-seconds/object: the actual currency paid is typically in proportion to this metric. Knowing an estimate of the number of objects in the annotation job, this will help \sysname  approximately estimate the cost of job. In \sysname each task is sent to multiple workers and some of the work is rejected while the rest is approved and paid. The total cost per task is thus the product of the number of people paid for each task times the time taken to complete a task. Knowing the number of objects per task in our experiments allows us to compute the person-seconds per object. By this metric (\figref{fig:accuracy}), image and video classification, and counting cost few tens of person-seconds/object while detection, tracking and segmentation require 160, 975 and xxx person-seconds respectively.
% Interestingly, tracking is faster than detection despite being slightly more expensive: this is because each tracking task can provide detection information in a few hundred frames at a cheaper cost. This is because, based on our experience, it easy to draw bounding boxes across frames of a video: not all frames need to be annotated since the annotation tool can interpolate between frames.


% \iffalse
% {
% In this section based on our experiments we also 
% \figref{fig:accuracy} also quantifies two other important metrics: the end-to-end \textit{latency} of collecting groundtruth as measured by the median latency to arrive at a fused result for a task, and the \textit{cost} to the requester in terms of number of \textit{approved} results per \satyam-task. These measures quantify the relative difficulty of the task. We find that the classification and counting tasks are an order of magnitude faster (7-10~hours) than localization and tracking (2-7~days). Tracking is the most expensive task requiring almost 12 workers' results to achieve acceptable fusion, followed by detection, with video classification being the cheapest. Interestingly, tracking is faster than detection despite being slightly more expensive: from our own experience, we have found it easy to draw bounding boxes across frames of a video: not all frames need to be annotated since the annotation tool can interpolate between frames.
% }\fi

% \subsection{Latency of Acquiring Groundtruth}
% \label{sec:evaluation:paramChoices}

% \begin{figure}
%   \centering
%   \includegraphics[width=\columnwidth]{figs/eval/ResultArrival.eps}
%   %\vspace*{-0.15in}
%   \caption{CDF of the First 500 Result Arrival Time}
%   \label{fig:accuracy}
% \end{figure}

% \begin{figure}
%   \centering
%   \includegraphics[width=\columnwidth]{figs/eval/BestParamAggregationTime.eps}
%   %\vspace*{-0.15in}
%   \caption{CDF of Aggregation Latency}
%   \label{fig:accuracy}
% \end{figure}


% For image classification, Detection, and Tracking, there is a substantial part of tasks for which \satyam finds it hard to extract a consensus. For those tasks, they often need to wait for more than enough results till \satyam conclude the confusion and select the majority as the result to terminate the task.   


\iffalse{
\begin{figure}
  \centering
  \includegraphics[width=\columnwidth]{figs/eval/adaptivePricing.eps}
  %\vspace*{-0.15in}
  \caption{Adaptive Pricing on Counting Task}
  \label{fig:adaptivePricing}
\end{figure}
}\fi

\iffalse{
\begin{figure}
  \centering
  \includegraphics[width=\columnwidth]{figs/eval/countingPDF1.eps}
  %\vspace*{-0.15in}
  \caption{Histogram of Time Per Counting Task over Different Datasets}
  \label{fig:countHist}
\end{figure}
\begin{figure}
  \centering
  \includegraphics[width=\columnwidth]{figs/eval/countingPDF2.eps}
  %\vspace*{-0.15in}
  \caption{Histogram of Time Per Counting Task over Different Datasets}
  \label{fig:countHist}
\end{figure}
}\fi

\subsection{Price Adaptation}
\label{sec:evaluation:priceAdaptation}

Figure~\ref{fig:timeCDF} is a CDF of the times taken by workers for all the various job categories in our evaluation. It clearly shows that the time taken to complete a task can vary by 3 orders of magnitude across our job categories.
% there is about 3 orders of magnitude difference among time taken to complete different kinds categories of tasks. 
Figure~\ref{fig:timeCDF_counting} depicts the pdf of the times taken for the same category -- counting task --  but for two different data sets \ie CARPK-1 and KITTI-Obj. 
KITTI-Obj has around 10 vehicles on average, and CARPK around 45 in each image, and the distribution of worker task completion times varies significantly across these datasets. (As an aside, both these figures have a long tail: we have seen several cases where workers start tasks but sometimes finish it hours later).

These differences motivate price adaptation. To demonstrate price adaptation in \satyam, we show the temporal evolution of price per HIT for CARPK-1 and KITTI-Obj in Figure~\ref{fig:adaptivePricing}. HIT price for KITTI-Obj converges within 200 results to the ideal target value (corresponding to median task completion time). CARPK-1 convergence is slightly slower due to its larger variability in task completion times (\figref{fig:timeCDF_counting}).

% The reason for the slow convergence in CARPK-1 is due to the larger variance in task completion times as depicted in Figure~\ref{fig:timeCDF_counting}. 

\subsection{Worker Filtering}
\label{sec:evaluation:workerFiltering}

To evaluate the efficacy of worker filtering ran \satyam with and without worker filtering turned on for each of the templates. \figref{tab:approvals} shows that for classification, counting and detection the approval rate is already quite high ranging close to 90\% and thus worker filtering brings about a modest increase in approval rates. For more involved tasks such as tracking and segmentation, the approval rates show a dramatic increase from 60\% to over 80\%. 


\subsection{Parameter Sensitivity}
\label{sec:evaluation:paramChoices}

\satyam's groundtruth fusion and result evaluation algorithms have several parameters and \figref{fig:accuracy} presents results for the best parameter choice. We have analyzed the entire space of parameters to determine the parameters that \satyam performance most crucially depends upon in terms of accuracy, latency and cost.

Image classification is sensitive only to two parameters: $n_{min}$, the minimum number of results before aggregation can commence, and $\beta$, the fraction determining the super-majority. The upper graph in \figref{fig:param:image_classification} shows how classification accuracy varies as a function of these two parameters. Because the cost and latency of groundtruth collection varies with parameters, the lower graph shows the cost (blue bars) and the latency (red bars) for each parameter choice. From this, we can see that when $n_{min}\ge 3$  and $\beta \ge 0.7$ the accuracy does not improve significantly, however, cost and latency increase. This indicates that $n_{min}=3$ and $\beta = 0.7$ are good parameter choices, with high accuracy, while having moderate cost and latency. \looseness=-1


%  (\figref{fig:param:video_classification}) (\figref{fig:param:counting})  (\figref{fig:param:localization}) (\figref{fig:param:tracking})
 
We have conducted similar analyses for video classification, counting, object detection (\figref{fig:param:localization}), segmentation, and tracking (\figref{fig:param:tracking}). Space constraints preclude a detailed discussion, but the key conclusions are:
(a) All job categories are sensitive to $n_{min}$, the minimum number of results before \satyam attempts to aggregate results;
(b) Each category is sensitive to one other parameter. For classification, this is the $\beta$ parameter that determines the super-majority criterion. For counting, it is the error tolerance $\epsilon$. For detection and tracking, it is $\eta_{cov}$, the fraction of corroborated groundtruth elements; and
(c) In each case, there exists a parameter settings at which provides good groundtruth performance at moderate cost and latency.


% Section~\ref{sec:evlaution:paramChoices} describes in detail, the various parameters chosen for each template and their sensitivity. 

% There are several parameters that must be chosen for aggregation in each template. 
% For each of the templates we performed a parameter sweep for all the parameters in the aggregation process and measure the sensitivity

\iffalse{
\begin{figure}
  \centering
  \includegraphics[width=0.9\columnwidth]{figs/eval/ParamSweep_ImageClassification.eps}
  %\vspace*{-0.15in}
  \caption{Accuracy, Latency and Cost: Image Classification}
  \label{fig:param:image_classification}
\end{figure}
}\fi

% \begin{figure}
%   \centering
%   \includegraphics[width=\columnwidth]{figs/eval/ParamSweep_VideoClassification.eps}
%   %\vspace*{-0.15in}
%   \caption{Accuracy, Latency and Cost: Video Classification}
%   \label{fig:param:video_classification}
% \end{figure}

% \begin{figure}
%   \centering
%   \includegraphics[width=\columnwidth]{figs/eval/ParamSweep_Counting.eps}
%   %\vspace*{-0.15in}
%   \caption{Accuracy, Latency and Cost: Counting}
%   \label{fig:param:counting}
% \end{figure}

% \begin{figure}
%   \centering
%   \includegraphics[width=\columnwidth]{figs/eval/ParamSweep_Detection.eps}
%   %\vspace*{-0.15in}
%   \caption{Accuracy, Latency and Cost: Localization}
%   \label{fig:param:localization}
% \end{figure}

% \begin{figure}
%   \centering
%   \includegraphics[width=\columnwidth]{figs/eval/ParamSweep_Tracking.eps}
%   %\vspace*{-0.15in}
%   \caption{Accuracy, Latency and Cost: Tracking}
%   \label{fig:param:tracking}
% \end{figure}


==> Satyam ArXiv/fusion.tex <==
%% Commented out
% \begin{figure*}[t]
% \centering
%   \begin{minipage}{0.66\columnwidth}
%   \centering
%   \includegraphics[width=0.95\columnwidth]{figs/MotivationAndAMTOverview/DetectionResult.eps}
%   %\vspace*{-0.15in}
%   \caption{Example Results of \satyam Detection from KITTI}
%   \label{fig:DetResult}
%  \end{minipage}
% \begin{minipage}{0.66\columnwidth}
%   \centering \includegraphics[width=0.95\columnwidth]{figs/MotivationAndAMTOverview/SegResult.eps}
%   %\vspace*{-0.15in}
%   \caption{Example Results of \satyam Segmentation from PASCAL}
%   \label{fig:SegResult}
% \end{minipage}
% \begin{minipage}{0.66\columnwidth}
%  \centering\includegraphics[width=0.95\columnwidth]{figs/MotivationAndAMTOverview/TrackingResult.eps}
%   %\vspace*{-0.15in}
%   \caption{Example Results of \satyam Tracking from KITTI}
%   \label{fig:TckingResult}
% \end{minipage}
% \end{figure*}

% \begin{figure}
%     \centering
%      \includegraphics[width=0.95\columnwidth]{figs/MotivationAndAMTOverview/DetectionResult.eps}
%   %\vspace*{-0.15in}
%   \caption{Example Results of \satyam Detection from KITTI}
%   \label{fig:DetResult}
% \end{figure}

% \begin{figure}
%     \centering
%      \includegraphics[width=0.95\columnwidth]{figs/MotivationAndAMTOverview/SegResult.eps}
%   %\vspace*{-0.15in}
%   \caption{Example Results of \satyam Segmentation from PASCAL}
%   \label{fig:SegResult}
% \end{figure}

% \begin{figure}
%     \centering
%      \includegraphics[width=0.95\columnwidth]{figs/MotivationAndAMTOverview/TrackingResult.eps}
%   %\vspace*{-0.15in}
%   \caption{Example Results of \satyam Tracking from KITTI}
%   \label{fig:TckingResult}
% \end{figure}

\begin{figure*}[t]
\centering
\begin{minipage}{0.65\columnwidth}
  \centering
  \includegraphics[width=0.9\columnwidth]{figs/QualityControl/QualityControlLoop}
  %\vspace*{-0.15in}
 \caption{Quality Control Loop in \sysname}
\label{fig:QualityControlLoop}
\end{minipage}
\begin{minipage}{0.6\columnwidth}
  \centering
  \includegraphics[width=0.8\columnwidth]{figs/QualityControl/Localization-Fusion-Example}
  \vspace{0.15in}
 \caption{Example groundtruth fusion in Multi-object Detection}
\label{fig:MultiObjectLocalizationFusion}
\end{minipage}
\begin{minipage}{0.65\columnwidth}
  \centering
  \vspace{3mm}
  \includegraphics[width=0.9\columnwidth]{figs/QualityControl/TrackingFusionExample}
  %\vspace*{-0.15in}
  %\vspace{-1mm}
 \vspace{6mm}
 \caption{Groundtruth fusion in Multi-object Tracking is a 3-D extension of Multi-object detection}
 
\label{fig:MultiObjectTrackingFusion}
\end{minipage}
\end{figure*}

\section{Quality Control}
\label{sec:fusion}

\sysname's quality control relies on the wisdom of the crowds~\cite{wisdom}: {\it when a large enough number of non-colluding workers independently agree on an observation, it must be ``close'' to the groundtruth}. To achieve this \sysname solicits groundtruth for the same image/video clip from multiple workers and only accepts elements of the groundtruth that have been \textit{corroborated} by multiple workers. For instance, in a detection task with several bounding boxes, only those, for which at least 3 workers have drawn similar bounding boxes, are accepted. 

\figref{fig:QualityControlLoop} depicts \satyam's quality control loop. One instance of the loop is applied to each \satyam-task. \sysname first sends the same task to  $n_{min}$ workers to obtain their results. $n_{min}$ depends on the job category and is typically higher for more complex tasks (described in more detail below). In the {\it groundtruth-fusion} step, \satyam attempts to corroborate and fuse each groundtruth element (\eg bounding box) using a job category specific groundtruth-fusion algorithm. If the fraction of corroborated elements in an image/video clip is less than the coverage threshold ($\eta_{cov}$), \sysname determines that more results need to be solicited and relaunches more HITs, one at a time. For some images/videos, even for humans, agreeing on groundtruth maybe difficult. For such tasks we place a maximum limit $n_{max}$ (20 in our current implementation) on the number workers we solicit groundtruth from. The task is marked ``aggregated'' and removed from the task list either if we reach the maximum limit or if the fraction of corroborated elements exceeds $\eta_{cov}$.

\subsection{Dominant Compact Cluster}
\label{sec:fusion:overview}

All the groundtruth-fusion algorithms in \sysname are based on finding the 
{\it Dominant Compact Cluster} (DCC) which represents {\it the set of similar results that the largest number of workers agree on}. If the number of elements in the dominant compact set is greater than $n_{corr}$, the groundtruth for that element is deemed as corroborated. 

\parab{Definition}
Suppose that $n$ workers have generated $n$ versions of the groundtruth $E_1,E_2,...,E_n$ for a particular element in the image/video (as in \figref{fig:MultiObjectLocalizationFusion} where each of the 4 workers has drawn bounding box around the orange car). 
For each job category, we define a distance metric $D(E_i,E_j)$ that is higher the more dissimilar $E_i$ and $E_j$ are. A fusion function $F_{fusion}(E_1,E_2,\cdots,E_k) = E_{fused}$ specifies how different versions of the groundtruths can be combined into one (\eg by averaging multiple bounding boxes into one).  
All {\it groundtruth-fusion} algorithms start by clustering ${E_1,E_2,\cdots,E_n}$ based on $D$ while guaranteeing that none of the elements of its cluster is farther than $\tau$ distance from the fused element \ie $D(E_{fused},E_k) < \tau$ for all $E_k$ within a cluster. $\tau$, the {\it compactness constraint}, ensures that the clusters do not have any results that are too dissimilar from each other. After the clustering, the cluster with the most number of elements is deemed the {\it dominant compact cluster} and  $E_{fused}$ computed over this cluster is deemed the cluster head. \looseness=-1

\parab{Greedy Hierarchical Clustering to find DCC}
Finding DCC is NP-Hard, so we use greedy hierarchical clustering. We start with $n$ clusters, the $i^{th}$  cluster having the one element $E_i$. At each step, two clusters with the closest cluster heads are merged, provided that the merged cluster does not violate the compactness constraint. The clustering stops as soon as clusters cannot be merged any longer.

\parab{Variations across different templates}
While finding the DCC is common across all groundtruth-fusion algorithms, the specific values and functions such as $n_{min}$, $D(E_i, E_j)$, $n_{corr}$, $F_{fusion}$, $\eta_{cov}$ and  $\tau$ are different for each fusion algorithm. In the rest of this section, we describe the various choices we use for these values and functions.

%Second, in order to measure whether groundtruth elements provided by two workers are similar, we define a similarity metric for each kind of groundtruth element e.g. similarly between two bounding boxes drawn by different workers. We then seek 

%in theconcluding collection of  ``enough'' workers to ensure coverage of all groundtruth elements.

%\satyam uses two key ideas in automating quality control for \satyam-jobs. The first idea applies to all job categories: \satyam sends each task to several independent non-colluding workers  The second idea is that it is possible to design a groundtruth-fusion algorithm for each specific \textit{job category} (as opposed to designing fusion algorithms for each specific job instance). A fusion algorithm for localization determines if a bounding box has been corroborated, and computes an \textit{aggregated} result that fuses  results from individual workers. Because there are relatively few categories, this approach of designing category-specific fusion algorithms scales well.

%Accordingly, there are two components to quality control in \satyam: a \textit{quality control loop} common to all job categories, and category-specific ground truth-fusion algorithms. We describe both in this section.

% \sysname sends the same task to several independent non-colluding workers, and uses {\it groundtruth-fusion} algorithms to piece together the correct parts from each worker to arrive at a high quality annotation. For example, in a localization task, some users might miss drawing bounding boxes around certain cars, miss-label them or draw incorrect bounding boxes. \sysname accepts specific parts of the groundtruth as ``correct'' only when they are corroborated by multiple workers e.g. 3 or more  workers draw a similar bounding box. If certain part of the groundtruth is not corroborated, the task is sent to more workers to allow for the possibility of corroboration. For example, in case there are many bounding boxes that have not received corroboration from 3 or more workers, \sysname will solicits more workers in the hope of corroborating these boxes. Finally, all parts of the groundtruth from every worker must be fused into one groundtruth. For example, no two workers will draw exactly the same boxes, and thus, different boxes must be intelligently combined into one.

\subsection{Fusion Details}
\label{sec:fusion:details}

%In these two job categories, workers are presented with an image/video with a set of classes, and asked to select the class that they believe the image/video belongs to. 
\parab{Image and Video Classification}
For this template, \satyam uses a super-majority criterion, selecting that class for which the fraction of workers that agree on the class exceeds $\beta \in (0,1)$ (we chose $\beta = 0.7$, \secref{sec:evaluation:paramChoices}). This is equivalent to the DCC algorithm with the distance function $D = 0$ if two workers choose the same category and $\infty$ if they do not, $\tau = 0$, and $n_{corr} = \beta n$, where $n$ is the number of results. 

%In these two job categories, workers are presented an image/video and asked to  count the number of instances of a certain event or object. 
\parab{Counting in Images/Videos}
Given $n$ counts, by $n$ workers, our goal is to robustly remove all the outliers and arrive at a reliable count. We use DCC for this, with  $D(C_i,C_j) = |C_i-C_j|$ where $C_i$ and $C_j$ are the counts from the $i^{th}$ and $j^{th}$ workers. $F_{fusion}$ is chosen as the average of all the counts. $\tau = \lfloor(\epsilon C)\rfloor$, where $C$ is the average count of the cluster, \ie two counts are deemed to be similar only if their deviation is less than $\pm \epsilon$ fraction of the average count. We chose $\epsilon = 0.1$ in our implementation. $n_{min}$ and $n_{max}$ are chosen to be 10 and 20 respectively (\secref{sec:evaluation:paramChoices}).

\parab{Object Detection in Images}
To provide intuition into the groundtruth fusion algorithm for this template we use the example in \figref{fig:MultiObjectLocalizationFusion}, where four workers have drawn bounding boxes around cars in an image. The $j^{th}$ bounding box drawn by the $i^{th}$ worker is represented by $B_{ij}$. A worker may not draw bounding boxes for all cars (\eg $W_2$ and $W_4$), and two different workers may draw bounding boxes on the same image in a different order (\eg $W_1$ draws a box around the red car first, but $W_3$ does it last). Furthermore, workers may not draw bounding boxes consistently: $W_3$'s box around the orange car is off-center and box $B_{11}$ is not tightly drawn around the red car. Our fusion algorithm, designed to be robust to these variations.
%uses the DCC algorithm for each object. 

\parae{Bounding Box Association}
Since different workers might draw boxes in a different order, we first find the correspondence between the boxes drawn by the different workers. In \figref{fig:MultiObjectLocalizationFusion}, this corresponds to grouping the boxes in the three sets {\small $G_1 =  \{B_{11},B_{22},B_{33}\}$, $G_2 =  \{B_{12},B_{31},B_{41}\}$} and, {\small $G_3 =  \{B_{13},B_{21},B_{32},B_{42}\}$} where each set has boxes belonging to the same car. We model this problem as a multipartite matching problem where each partition corresponds to the bounding boxes of a worker, and the goal is to match bounding boxes of each worker for the same car.

To determine the matching, we use a similarity metric, {\it Intersection over Union (IoU)}, between two bounding boxes, which is the ratio of intersection of the two bounding boxes to their union. Since the matching problem is NP-Hard, we use an iterative greedy approach. For a total of $N$ bounding boxes, we start with $N$ sets with one bounding box per set. At each iteration, we merge the two sets with the highest average similarity  while ensuring that a set may have only one bounding box from a partition. The algorithm terminates when there are no more sets that can be merged. In the end, each set corresponds to all the boxes drawn by different workers for one distinct object in the image.

%At each step, the a new bounding box is added to a set with the most similar %boxes (smallest mean IoU) while ensuring that no partition has two bounding %boxes by the same worker. The process terminates when there are no more %bounding bowhich matches box-pairs in decreasing order of similarity. 

% If there were a total of $N$ bounding boxes drawn, we start with $N$ bounding box groups where each group corresponds to a single bounding box. In each   

\parae{Applying groundtruth-fusion on each object}
Once we know the set of bounding boxes that correspond to each other, we can use DCC for fusion. 
Let bounding box {\small $B_i = \left<x_i^{tl},y_i^{tl},x_i^{br},y_i^{br}\right>$} where {\small $(x_i^{tl},y_i^{tl})$ and $(x_i^{br},y_i^{br})$} are the top left and bottom right pixel coordinates respectively. We choose {\small $D(B_i,B_j) = \max(|x_i^{tl}-x_j^{tl}|$,$|y_i^{tl}-y_j^{tl}|$,$|x_i^{br}-x_j^{br}|$, $|y_i^{br}-y_j^{br}|)$, $n_{corr} = 3$, $\tau = 15$} (pixels), {\small $n_{cov} = 0.9$, $n_{min}=5$, $n_{max}=20$}. The fusion-function $F_{fusion}$ generates a fused bounding box as the average of each of top-left and bottom-right pixel coordinates of all the bounding boxes being fused.
Thus, in order to be similar, none of the corners of the boundaries must deviate by more than $\tau$ pixels along the $x$ or $y$ axis. The minimum number of workers to corroborate each box is 3 and 90\% of the boxes need to corroborated before the quality control loop terminates. We arrived at these parameters through a sensitivity analysis (\secref{sec:evaluation:paramChoices}).

% In Section Section~\ref{sec:eval:xxx} we discuss how these choices were made.


% \iffalse
% {
% We choose $D(B_1, B_2)$ as the maximum of difference between each pixel coordinate
% The output of this step is a \textit{fused} bounding box that aggregates boxes within each group $G_i$. To do this, we perform hierarchical clustering over the entire bounding box group using IoU as our metric to ensure that the most similar bounding boxes are grouped together. Suppose a group contains $k$ bounding boxes. Consider a subset $S$ containing $k'$ of these boxes. Now, let box $B_{m,S}$ be the \textit{mean} bounding box of subset $S$: it is defined by taking the centroid of the top-left and bottom-right corners of the $k'$ bounding boxes. Of the $k'$ boxes, let $k''$ be the number of boxes whose IOU with respect to $B_m$ is at least $IOU_{min}$. Then, we say that the fused bounding box for group $G_i$ is that $B_{m,S}$ whose $k''$ is the largest. Furthermore, we require $k''$ to be greater than $n_{corr}$: this condition ensures a minimal number of corroborations for a box. Rather than evaluate all possible subsets $S$, we construct these subsets greedily, starting from $k$ singleton sets and merging them at each step if the $IOU_{min}$ criterion can be met.


% % For a set of bounding boxes, we define the mean bounding box as that having the average of the top right and bottom left corners. Then we select the largest bounding box group that satisfies the maximum IOU deviation criterion -- none of the bounding boxes should have an IoU less than the IoU threshold $IOU_{min}$. The final bounding box is then the bounding box mean bounding box of this largest set.The largest bounding box set must have at least $n_{corr}$ bounding boxes in order to be deemed as valid i.e, it has to be corroborated by at least $n_{cor}$ workers (3 in our implementation).

% \parab{Determining if more worker inputs are needed}
% The fusion step may not output a fused bounding box if not enough or operations exist. If, for a given image, $f_{min}$ or more fraction of box groups remain uncorroborated after the fusing process, the the task is deemed unfinished and more workers are solicited. %We chose $f_{min}$ as 0.8 in our implementation.
% }\fi

% \parab{Fusing the category labels} Within each bounding box group we use the algorithm of \secref{sec:fusion:classification} to fuse object class labels. This step may also be inconclusive, in which case \satyam may solicit more workers for the task.
% \iffalse{
% \parab{Parameter choices}
% Our algorithm contains three parameters ($n_{corr}$, $IoU_{min}$, $f_{min}$) designed to achieve accurate fusion in the face of human error, while permitting forward progress in cases where  localization is difficult even for humans. In \secref{sec:eval}, we discuss how to set these parameters.
% }\fi

\parab{Object Segmentation in Images}
The fusion algorithm used for image segmentation is almost identical to that used for multi-object detection except that bounding boxes are replaced by segments: arbitrary collections of pixels. Thus, while associating segments instead of bounding boxes, the IoU metric is computed by considering individual pixels common to the two segments. For $F_{fusion}$, a pixel is included in the fused segment only if it was included in the annotations of at least 3 different workers. We use $\tau = 1/0.3$, $n_{corr}= 3$, $n_{min}=10$, $n_{max}=20$ and $\eta_{cov}=0.9$. % For $F_{fusion}$

\parab{Object Tracking in Videos}
Fusion algorithm for multi-object tracking simply extends that used for multi-object detection to determine a fused \textit{bounding volume}, a 3-D extension of bounding box  (as shown in Figure~\ref{fig:MultiObjectTrackingFusion}). We extend the definition of IoU to a bounding volume by computing and summing intersections and unions over each frame, deemed {\it 3D-IoU}. %The DCC-based groundtruth fusion uses the inverse of this extended IoU for the distance function $D$ as well. 
For $F_{fusion}$, we average the bounding boxes across users at each frame independently; this is because different workers may start and end the track at different frames.
We use {\small $\tau = 1/0.3$, $n_{corr}= 3$, $n_{min}=5$, $n_{max}=20$} and {\small $\eta_{cov}=0.9$}.

%the same two step process as the algorithm of %\secref{sec:fusion:localization}, with two differences. First,  Second, to %compute the \textit{mean bounding volume}, 

% \iffalse{
% Based on the observation that reliable workers are likely to have similar counts (defined as counts that deviate by no more than $\epsilon$ from the mean), we use a hierarchical clustering approach (similar to fusing bounding boxes in \secref{sec:fusion:localization}) to identify the largest subset of reliable workers. Our algorithm starts with each count in a separate cluster, and merges two clusters if each worker's count in the combined cluster is within $\epsilon$ of the mean. Clustering terminates either when a single cluster remains or no two clusters can be merged. As before, we require each cluster to have $n_{corr}$ results, failing which we recruit more workers.
% }\fi
% Our scheme is based on the idea that groups of workers sometimes incorrectly count by missing some objects in certain parts of the image/video and thus worker's counts will occur in clusters with a small deviation in counts within each cluster. Thus, our approach is to first define a maximum tolerable deviation for each cluster as a fraction $\epsilon$ ($\pm$ 10\% in our implementation) of the average count within each cluster. We perform hierarchical clustering where starting with $n$  clusters (each comprising of one count), at each step, the two clusters with closest average count values are combined if the average count of combined cluster does not violate the  $\epsilon$ deviation criterion. The clustering terminates either when $k=1$ or if no two clusters can be merged. Finally, the cluster with the highest count that has its cardinality greater than a threshold (3 in our implementation) is deemed the winning cluster and its average chosen as the final count.

\subsection{Result Evaluation}
\label{sec:fusion:resultEvaluator}

After all the results for a task have been fused, \satyam \textit{approves} and pays or \textit{rejects} each worker's HIT (\secref{sec:payments}). 

% they are compared against the aggregated (fused) groundtruth, to determine whether or not the worker performed satisfactorily or not. This is necessary to decide whether or not the worker deserves to be paid. 

For image and video \textit{classification}, \satyam approves all HITs in which the worker's selected class matches that of the aggregated result. When no class label achieves a super-majority (\secref{sec:fusion:details}), it ranks all classes in descending order of the number of workers who selected them, then chooses the minimum number of categories such that the combined number of workers that selected them is a super-majority, and approves all their HITs.
For \textit{counting}, \satyam approves each worker whose counting error is within $\epsilon$ of the fused count (\secref{sec:fusion:details}).
For object \textit{detection, segmentation and tracking}, \satyam approves each worker whose work has contributed to most of the objects in the image/video. Specifically, \satyam approves a worker if the bounding boxes generated by the worker were in more than half of the dominant compact clusters (\secref{sec:fusion:details}) for objects in the image.


% for each worker,  count the number of objects a certain worker's bounding boxes contributed to i.e. was used in computing the final bounding box. If this number is greater than a certain fraction (50\% in our implementation) more than the total number of objects in the image/object we consider the worker as deserving and approve (pay) their work.


==> Satyam ArXiv/ground_truth.tex <==
\begin{figure*}[h]
  \centering
  \begin{minipage}{2.1in}
\includegraphics[width=1.9in]{figs/MotivationAndAMTOverview/MotivationBeforeAfterFineTuning}
  \vspace*{-0.15in}
 \caption{Improvement of performance with fine tuning}
\label{fig:MotivationYoLoPerformance}
\end{minipage}
\begin{minipage}{2.1in}
  \includegraphics[width=1.9in]{figs/MotivationAndAMTOverview/MotivationExampleYoLoBefore}
  \vspace*{-0.15in}
 \caption{Example of YoLo's output before fine-tuning (from data set $Cam1$) }
\label{fig:MotivationYoLoBefore}
\end{minipage}
\begin{minipage}{2.1in}
\includegraphics[width=1.9in]{figs/MotivationAndAMTOverview/MotivationExampleYoLoAfter}
  \vspace*{-0.15in}
 \caption{Example of YoLo's output after fine-tuning (from data set $Cam1$)}
\label{fig:MotivationYoLoAfter}
\end{minipage}
\end{figure*}

\section{Obtaining Groundtruth using AMT}
\label{sec:gt}

In this section we first motivate the need for using crowdtasking systems such as AMT for machine vision based systems and then explain the various challenges involved in obtaining groundtruth. To guide us we we use a practical traffic video surveillance system as an example. 

\subsection{Need for Groundtruth}
\label{sec:gt:NeedForFineTuning}
The performance of ML systems is only as good as the data they are trained on.
There are several publicly available pre-trained ML models for various machine vision scenarios that are trained on benchmark data sets. However, directly employing these ML models in the field often results in poor accuracy, since the nature and conditions of the images in the field are often very different from those in the benchmark data sets. A common approach is to start with a publicly available ML model, but then follow it up with a fine-tuning step where the model is trained further on actual data from the field. In many practical deployments, testing and fine-tuning becomes a periodic activity to keep adapting to changing conditions and to maintain performance guarantees.

In order to provide the reader with an intuition we leverage a real life example -- a vision system that locates cars in traffic video surveillance images. We obtain HD quality images from four busy traffic intersections in two  prominent U.S. cities. Images are collected between 7:00 A.M to 7:00 P.M over a week (7 days) at one minute intervals to cover all the different conditions in the scene -- a total of 5000 images/camera (20000 images). We use a popular deep neural network, YOLO~\cite{yolo}, that generates bounding boxes for objects of interest (cars). We obtain groundtruth bounding boxes for the cars in each images using \satyam. The data for each camera is partitioned into 20\% testing and 80\% training data sets. 

We start with a publicly available pretrained ML model YoLo-Coco -- YoLo trained on the CoCo data set~\cite{XXX}. We also then fine-tune YoLo-CoCo  specifically each camera, by retraining its last-layer (a common practice) using the training data for that camera. As depicted in Figure~\ref{fig:MotivationYoLoPerformance},  YoLo-CoCo performs poorly on all the four cameras with a precision of under 50\%. This poor performance occurs because the characteristics of the specific camera footage e.g. angle, background scenery etc are often very different from that in the training images in the CoCo dataset. After fine-tuning, (YoLo-FineTuned), there is a dramatic improvement in accuracy (> 80\%) for each camera. Figures~\ref{fig:MotivationYoLoBefore} and~\ref{fig:MotivationYoLoAfter} show an example of YoLo output before and after the fine-tuning. 


\subsection{Labling Effort}
\label{sec:gt:effort}
In order to fine tune YoLo, the groundtruth required for each image is the set of all bounding boxes for each car (specified by the pixel coordinates of their top left and right bottom corners). With about 15-25 cars per image, the process of drawing a box around each object takes on average 90 seconds per image and amounts to approximately 125 man-hours per camera. This example demonstrates how even this relatively ``small scale'' experiment requires a huge manual effort in terms of groundtruth annotation.

\subsection{AMT Overview and Terminology}
\label{sec:gt:Need}
AMT provides on-demand access to a pool of workers that can potentially help with the groundtruth annotation effort. However, one has very little/no direct control over these workers and they are free to choose among the several thousands of jobs in the AMT platform based on their preferences. 

\parab{Human Intelligence Task (HIT)} HIT is the minimum unit of work for which a worker is paid for upon finishing it "acceptably". HITs appear as a webpages to the worker and are typically tasks that can be done within the confines of a browser. In our example, one HIT would comprise a worker drawing boxes around all the cars in a single image. 

\parab{Requesters} are users who create HITs and are responsible for accepting (paying) or rejecting (not paying) the work performed by the workers.

\subsection{Challenges in Using AMT}
\label{sec:gt:challenges}

In this section we describe the various steps and challenges involved in using AMT for groundtruth collection.

\parab{Creating Web-UI HITs}
The first step to using AMT is to creating a web application that displays a specific image/video clip equipped with a UI and appropriate instructions that makes it easy for untrained workers to annotate groundtruth easily and accurately. Design of these UIs can be extremely challenging and there exists a large body of research that focuses on UI design for various tasks e.g.~\cite{VATIC}. Often the expertise and effort needed to develop a web-UI is a deterrent to using crowdtasking platforms. 
 
\parab{Quality Control} 
Workers in AMT are untrained and may not generate a good annotation. In our traffic surveillance example, workers may miss drawing boxes around cars either due to negligence, inexperience with the UI or simply lack of interest. In our experience, a significant fraction of the results from the workers are always incorrect, especially for more sophisticated machine vision applications. Thus, the onus of determining which results are acceptable solely lies on the requesters, who have to typically inspect the results manually. For incorrect results, these annotation tasks may have to be resent to more workers. For large data sets this manual intervention, quickly becomes unscalable. 

\parab{HIT Management -- Launching and Payments} 
A HIT is typically launched for each image and launching tens of thousands of HIT annotations requires automation using AMT web service APIs. Further, when some annotations are unacceptable, these must be identified and re-launched to more workers. The requester is also responsible identifying and paying the deserving workers while rejecting the rest. This is once again a manual process and does not scale. 



==> Satyam ArXiv/implementation.tex <==
\section{Implementation on Azure}
\label{sec:impl}
\sysname has been implemented on Azure and written primarily using C#, javascript and the ASP .Net framework comprising a total of XXX lines of code. As described


Various components
\begin{itemize}
    \item Templates – description and examples of where they are used
    \item Template to Tasks
    \item Amazon HIT Launching logic
    \item Fusion, Consensus Algorithms and Relaunching
    \item Accept Reject Criterion and Paying
    \item Results saving
\end{itemize}

==> Satyam ArXiv/overview.tex <==
\section{\sysname Overview}
\label{sec:overview}

\sysname is designed to minimize friction for non-expert users when collecting groundtruth for ML-based machine vision systems. It uses AMT but eliminates the need for users to develop complex Web-UIs or manually intervene in quality control or HIT management.

% \sysname achieves this by leveraging human workforce provided by AMT crowdtasking platform while automating its three challenging aspects Section~\ref{sec:gt:challenges} -- Web-UI  generation, HIT Management and Quality Control. In this section we provide a high level overview of the various components of \sysname that automate these three challenges.

% \begin{figure}[h]
%   \centering
%   \includegraphics[width=1.6in]{figs/Overview/JobsTasksHits}
%  \caption{\sysname's jobs, tasks and HITs}
%  \label{fig:State-Transitions}
% \end{figure}

% \subsection{Design Goals}
% \label{sec:overview:functioning}

%\satyam's design is guided by five goals.

\subsection{Design Goals}
\label{sec:overview:design_goals}
We now briefly describe the key design goals that shaped the architectural design of \satyam.

\parab{Ease of use} \satyam's primary design goal is \textbf{\textit{ease of use}}. \satyam users should only be required to provide a high-level declarative specification of ground-truth collection: what kind of ground-truth is needed (\eg class labels, bounding boxes), for which set of images/videos, how much the user is willing to pay, \etc \satyam should not require user intervention in designing UIs, assessing result quality, or ensuring the appropriate HIT price, \etc, but must perform these automatically. 

\parab{Scalability} \satyam will be used by multiple concurrent users, each running several different ground-truth collection activities. Each activity in turn might spawn several tens of thousands of requests to workers, and each request might involve generating web user interfaces, assessing results, and spawning additional requests, all of which might involve significant compute and storage. 


\parab{Asynchronous Operation} Because \satyam relies on humans in the loop, its design needs to be able to \textbf{\textit{tolerate large and unpredictable delays}}. Workers may complete some HITs within a few seconds of launch, or may take days to process HITs. 

\parab{Evolvability} In designing algorithms for automating ground truth collection, \satyam needs to take several design dimensions into account: the requirements of the user, the constraints of the underlying AMT platform, variability in worker capabilities, and the complexity of assessing visual annotation quality. These algorithms are complex, and will evolve over time, and \satyam's design must accommodate this evolution.

% \satyam uses several algorithms and web-UIs in its components that can be improved in the future for developers. Consequently, \sysname's architecture is designed to be evolvable; each component is made of modules that conform to well defined interfaces and can be replaced by more accurate or efficient ones in the future.

\parab{Extensibility}
ML for machine vision is rapidly evolving and future users will need new kinds of groundtruth data which \satyam must be able to accommodate.

\looseness=-1 

% \sysname makes it easy for a layperson to launch groundtruth collection tasks by eliminating the need for developing complex Web-UIs for the annotation. Instead it provides the user with a suite of Web-UI templates. The user need only to select one among them, then customize it by specifying a handful of parameters specific to the required groundtruth and press the submit button. The templates are designed based on the observation that the Web-UI requirements of most groundtruth collection tasks for machine vision applications fall into one among a few standard templates. 


% \parab{Scalability} \satyam will be used by multiple concurrent users, each running several different ground-truth collection activities. Each activity in turn might spawn several tens of thousands of requests to workers, and each request might involve generating web user interfaces, assessing results, and spawning additional requests, all of which might involve significant compute and storage. \satyam should be designed to scale to tens or hundreds of large concurrent groundtruth collection activities.

% Consequently, scalability is a key design goal in \sysname. \sysname is designed as a set of components in a pipeline, each of which performs one specific step in the process of groundtruth collection (\figref{fig:Satyam-Components}). Each component can be run as an independent process and is highly parallelizable to the granularity of a single task. 

% \parab{Asynchronous operation} 
% Because \satyam relies on humans in the loop, its design needs to be able to tolerate large and unpredictable delays. Workers may complete some HITs within a few seconds of launch, or may take days to process HITs. \looseness=-1

% To accommodate this inherent asynchronous nature, each component in \sysname is designed to start up periodically, read all required information from one or more tables and then write/edit/delete records in one or more tables for other components to use when they start. Thus, each component may be run as an Azure function or Amazon Lambda as frequently as required.

% \parab{Evolvability} In designing algorithms for automating ground truth collection, \satyam needs to take several design dimensions into account: the requirements of the user, the constraints of the underlying AMT platform, variability in worker capabilities, and the complexity of assessing visual annotation quality. These algorithms are complex, and will evolve over time, and \satyam's design must allow this evolution.

% \satyam uses several algorithms and web-UIs in its components that can be improved in the future for developers. Consequently, \sysname's architecture is designed to be evolvable; each component is made of modules that conform to well defined interfaces and can be replaced by more accurate or efficient ones in the future.

% \parab{Extensibility}
% ML for machine vision is rapidly evolving and future users will need new kinds of groundtruth data which \satyam must be able to accommodate.

% As described later in this section, \sysname is designed to be extensible to allow new kind of groundtruths to be collected without having to change most of its core components but simply adding more modules or web-UIs.

\begin{figure}[t]
\centering
\begin{minipage}{0.9\columnwidth}
   \centering\includegraphics[width=0.7\textwidth]{figs/Overview/JobsTasksHits}
   %\vspace*{-0.15in}
   \caption{\sysname's jobs, tasks and HITs}
   \label{fig:JobsTasksHits}
\end{minipage}
%\vspace*{-2mm}
\end{figure}

\begin{figure*}[t]
  \centering
  \begin{minipage}{0.75\columnwidth}
%   \centering\includegraphics[width=0.95\textwidth]{figs/Overview/JobsTasksHits}
%   %\vspace*{-0.15in}
%   \caption{\sysname's jobs, tasks and HITs}
%   \label{fig:State-Transitions}
    \centering
    \includegraphics[width=0.95\textwidth]{figs/MotivationAndAMTOverview/Coverage.pdf}
    \caption{\satyam Job Categories}
    \label{fig:templates}
  \end{minipage}
  \begin{minipage}{1.25\columnwidth}
  \centering\includegraphics[width=0.90\textwidth]{figs/Overview/Satyam-Components.pdf}
  %\vspace*{-0.15in}
  \caption{Overview of the \sysname's components}
  \label{fig:Satyam-Components}
  \end{minipage}
  \vspace*{-2mm}
\end{figure*} 

% \subsection{Jobs, Tasks and HITs}
% \label{sec:overview:jobs_tasks_hits}



\subsection{\satyam Abstractions}
\label{sec:overview:abstractions}
\satyam achieves ease of use and asynchronous operation by introducing different abstractions to represent logical units of work in groundtruth annotation (depicted in Figure~\ref{fig:JobsTasksHits}).

\parab{\satyam-job} Users specify their groundtruth collection requirements at a high-level as a \textbf{\textit{\satyam-job}}, which has several parameters: the set of images/video clips, the kind of groundtruth desired (\eg bounding rectangles for cars), payment rate (\$/image or  \$/hour), the AMT requester account information to manage HITs on the user's behalf, \etc At any instant, \satyam might be running multiple \satyam-jobs.

\parab{\satyam-tasks} \satyam renders jobs to \textbf{\textit{\satyam-tasks}}, which represent the smallest unit of groundtruth work sent to a worker. For example, a \sysname-task might consist of a single image in which a worker is asked to annotate all the bounding rectangles and their classes (\secref{sec:intro}), or a short video clip in which a worker is asked to track one or more objects. A single \sysname-job might spawn hundreds to several tens of thousands of \sysname-tasks.  

\parab{HIT} A \textbf{\textit{HIT}} is an AMT abstraction for the smallest unit of work for which a worker is paid. \satyam decouples HITs from \satyam-tasks, for two reasons. First, \satyam may batch multiple \satyam-tasks in a HIT. For example, it might show a worker 20 different images (each a different \sysname-task) and ask her to classify the images as a part of a single HIT. Batching increases the price per HIT thereby incentivizing workers more, and also increases worker throughput. Second, it allows a single \satyam-task to be associated with multiple HITs, one per worker: this permits \satyam to obtain groundtruth for the same image from multiple workers to ensure high quality results. \looseness=-1

% {\bf How is a HIT different from a \sysname-Task?} HIT is the smallest work unit that a worker is paid for in the context of AMT. A HIT might sometimes  
%  require a worker to work on multiple \sysname-tasks. For example, a worker might be shown 20 different images (each a different  \sysname-task) and asked to classify them as a part of a single HIT. This bunching is often desirable as workers have higher throughput when they perform many small tasks in rapid succession rather than individually and prefer to work on HITs that pay higher per HIT. Further, since \sysname obtains groundtruth for the same task from multiple workers, a single \sysname-task might be a associated with multiple different HITs, one for each worker. 
 
\subsection{\satyam Architecture}
\label{sec:overview:architecture}
\sysname is architected as a collection of components (\figref{fig:Satyam-Components}) each implemented as a \textit{cloud function} (\eg an Azure function or an Amazon lambda) communicating through persistent storage. This design achieves several of \satyam's goals. Each component can be scaled and evolved independently. Components can be triggered by users requesting new jobs or workers completing HITs and can thereby accommodate asynchronous operation. Finally, only some components need to be modified in order to extend \satyam to new types of ground truth collection.

\satyam's components can be grouped into three high-level functional units, as shown in \figref{fig:Satyam-Components}: {\it Job Rendition}, {\it Quality Control} and {\it HIT Management}. We describe these components, and their functional units, in the subsequent sections.

 \parab{Job Rendition} 
 This functional unit raises the level of abstraction groundtruth collection (Section~\ref{sec:templates}). It is responsible for translating the user's high level groundtruth collection requirements to AMT HITs and then compiling the AMT worker results into a presentable format for users. Users primarily interact with the {\it Job-Submissions Portal}~\cite{satyamportal_website} where they submit their groundtruth collection requirements. Submitted jobs are written to the {\it Job-Table}. Based on the job descriptions in the Job-Table, the {\it Pre-processor} may perform data manipulations such as splitting videos into smaller chunks. The {\it Task Generator}  decomposes the \sysname-job into \sysname-tasks, one for each image/video chunk. The {\it Task Portal} is a web application that dynamically renders \sysname-tasks into web pages (based on their specifications) displayed to AMT workers. Finally, {\it Groundtruth Compilation} assembles the final results from the workers for the entire job and provides them to \sysname users as a JSON format file.

 \parab{Quality Control}
 AMT workers are typically untrained in groundtruth collection tasks and \sysname has little or no direct control over them. Further, some of the workers might even be bots intending to commit fraud~\cite{mturk-spam}. The quality control components are responsible for ensuring that the groundtruth generated by \sysname is of high quality. In order to achieve this, \sysname sends the same task to multiple non-colluding workers and combines their results. The {\it Result Aggregator} identifies and fuses the ``accurate parts'' of workers' results while rejecting the ``inaccurate parts'' using {\it groundtruth fusion algorithms} described in \secref{sec:fusion}. For certain tasks, the Aggregator might determine that it requires more results to arrive at a conclusive high quality result. In that case, it presents the task to more workers until a high quality groundtruth is produced. The {\it Results Evaluator} compares fused results with the individual worker's results to determine whether the worker performed acceptably or not and indicates this in the {\it Result-Table}. \looseness=-1

\parab{HIT-Management} These components directly interact with the Amazon AMT platform and manage HITs through their life-cycle (\secref{sec:payments}). The {\it HIT Generator} reads the task table and launches HITs in AMT and always ensures that there are no unfinished tasks with no HITs. It is also responsible for {\it adaptive pricing} -- adaptively adjusting the HIT price by measuring the median time to task completion, and {\it worker filtering} -- ensuring that under-performing workers are not recruited again.  The {\it HIT Payments } component reads the results table and pays workers who have completed a task acceptably, while rejecting payments for those who have not. The {\it Task Purge} component removes tasks from the task table that have already been aggregated, so that they are not launched as HITs again and the {\it HIT Disposer} removes any pending HITs for a completed job. 

% \iffalse{
% \sysname must convert the high level groundtruth requirements of its users into AMT HITs. Users interact with \sysname through a web-portal -- the {\it job submissions portal}, where they specify and submit groundtruth collection jobs. At the job sumbissions portal, a user begins by selecting and customizing a suitable \textit{groundtruth template} from a suite of available templates, each designed for generating a Web-UI for a specific kinds of groundtruth annotation (described in detail in Section~\ref{sec:templates}). 
% Submitted jobs are stored in the {\it Job Table}. The \sysname pre-processor reads the job table for freshly submitted jobs and pre-processes the videos/images e.g. breaks large videos into smaller manageble chunks. The \sysname task generator, then 

% Translating  user's groundtruth collection requirements to Amazon HITs, Ensuring that it can generate high quality groundtruth from annotations done by workers and HIT management -- quality control Ensuring that quality control 

% \parab{Job-Submission Portal and Customizable Templates}
% The job-submission web portal is the primary interface through which users interact with \satyam.  For example, if the desired groundtruth is bounding boxes around cars and pedestrians in a traffic surveillance image, the user would select the  {\it multi-object localization} template. From this template, \satyam auto-generates a web-UI (described below) that allows a worker to draw and edit bounding boxes on the displayed image and specify the type of object by selecting on a radio button list. These templates were chosen to cover the most popular kinds of groundtruth data used in machine vision applications (\secref{sec:templates}).  

% After selecting a template, a user customizes it by specifying various parameters such as the list of objects/classes of interest with their descriptions, the price she intends to pay, a cloud storage source that contains the images or videos \etc and then submits the job. After she submits a job to the \sysname job submission portal~\cite{xxx}, \satyam stores the entire specification of the job is stored in the {\it \sysname Job-Submission Table} and identifies it by a globally unique identifier, the \textit{Job-GUID} (\secref{sec:impl}). 

% \parab{\satyam Pre-Processor}
% The pre-processing component reads the Job-Submission table for freshly submitted jobs to see if there are any freshly submitted jobs and performs the necessary preprocessing on the images/video clips. For example, breaking large video clips into smaller managable chunks. Once the images/videos of a job are preprocessed, it is deemed ready for the task-generation component. 

% \parab{\sysname Task Generation}
% This component checks the \sysname Job-Submission Table to see if there are any freshly preprocessed jobs. It then decomposes jobs into \sysname-tasks and stores all the \sysname-task definitions in the \textit{\sysname-task table}. A \sysname-task definition has all the necessary metadata to perform the specific task \eg the URI specifying the image/video clip, the associated job GUID, as well as the number of attempts and completions of a task. 

% \parab{\sysname HIT Generator}
% This component creates HITs in AMT using the (web-service API that AMT provides~\cite{mturk_sdk}) and associates these HITs with an entry in the {\it HIT Table} (which also contains pricing metadata, as well as job/task identification). The HIT generator ensures that every unfinished task in the \satyam-task table has at least one HIT associated with it in AMT. 

% \parab{\sysname Task Web-UI Portal}
% An AMT worker sees HITs listed by the title of the template and the price promised for completing the HIT. (At any given instant, \satyam can be running multiple \satyam-jobs for each supported template). When the worker \textit{accepts} a HIT, she is directed to the \satyam Task Web-UI Portal, which dynamically generates a web page containing one or more \satyam-tasks. The generated web page appears as an IFrame within the AMT website. Each time the worker submits results of the HIT, these are entered into a {\it Results Table}. 

% When dynamically generating the web page, \satyam needs to determine which \satyam-tasks to present to the worker. Listing HITs only by task portal and by price allows delayed binding of a worker to \satyam-tasks. \satyam uses this flexibility to (a) achieve uniform progress on \satyam-tasks and (b) avoid issuing the same task to the same worker. When a worker picks a HIT for template $T$ and price $p$, \satyam selects that \satyam-task with the same $T$ and $p$ which has been worked upon the least (using a random choice to break ties). Furthermore, \satyam can determine, from the task table, if the worker has already worked on this task (\satyam may present the same task to multiple workers to improve result quality, \secref{sec:fusion}). In this case, \satyam selects another \satyam-task to avoid assigning the same worker twice to the same task. More generally, a single HIT may present multiple \satyam-tasks, so \satyam repeats this procedure until enough tasks have been assigned to the HIT.

% % When a worker
% % These webpages are dynamically generated based on the task definitions obtained from the \sysname-task table. To ensure that the same worker does not work on the same task again and again, the tasks with the same HIT price to dispatched in prioritized random order from the task table, where a task is chosen randomly from the highest priority tasks. In our current implementation, to ensure broad coverage, tasks that have been worked upon by workers the least are given the highest priority. The generated web page appears as an IFrame within the AMT website. Each time the results of a task are submitted by the user, they are populated into the {\it Results Table}. 

% \parab{\sysname Result Aggregator and Quality Control}
% To be robust to spammers and careless workers, \satyam dispatches each \sysname-task to multiple workers (HITs). Its Result Aggregator fuses results from the Result Table to produce a single consistent high quality result using {\it groundtruth-fusion} algorithms (\secref{sec:fusion}) and stores these in the {\it Aggregated Results Table}. The groundtruth-fusion algorithms may not be able to arrive at an aggregated result if insufficient HIT results are available. Arrival of new results triggers the Result Aggregator. Occasionally, a task may not be aggregatable if not enough workers have chosen to work on it, or their annotations are incorrect (\secref{sec:fusion}).

% % this reason,  new results arrive, the Result Aggregator is invoked
% % The attempt may lead to a failure i.e. conclusion that more results are required to arrive at consistent picture or a success i.e. an aggregated result. 

% \parab{\sysname Result Evaluator} 
% \satyam needs to assess each worker's result to decide whether or not the work deserves payment. AMT permits HITs to be rejected, and \satyam uses this to discourage spammers and careless workers (see also \secref{sec:learnings} for a more detailed discussion). For every aggregated result for a \satyam-task, \satyam's Result Evaluator checks every HIT result from the Results Table, and determines (\secref{sec:payments}) whether the result was \textit{accepted} or \textit{rejected}. The key intuition behind this determination is that, because \satyam has results from multiple workers, its fusion algorithms produce a consensus result, and workers that deviate significantly from this consensus need not be paid.

% \parab{\sysname HIT Payments.} A single HIT may include multiple \satyam-tasks. \satyam's HIT Payments component computes the fraction of \textit{accepted} results across all of these tasks. If this fraction is above a threshold (see \secref{sec:learnings} for a discussion on how to set the threshold), the worker is paid.

% % is responsible for paying workers who have completed their HITs acceptably. In order to achieve this, it reads checks all the Results corresponding to a HIT to check what fraction of them were accepted. If this fraction is greater than an "acceptable" threshold, the worker is paid for this HIT. We use 70\% as the threshold in our current implementation. 

% % This component periodically checks for unevaluated results in the Results Table. Upon finding them, it then looks for the corresponding aggregated result in the Aggregated Results Table. If not aggregated result is found, then the result remained unassessed. Upon finding an aggregated result, the result is compared to the aggregated result to find if the worker performed "acceptably" and then the result is deemed {\it accepted} or {\it rejected} (details in Section~\ref{sec:pricing}).    

% \parab{\sysname Task Purge.}
% This component reads the Aggregated Results Table and removes all the completed \sysname-tasks from the Task Table ensuring that these tasks no longer show up in any future HITs. 

% \parab{\sysname Groundtruth Compilation.}
% Once all the tasks corresponding to a job have been purged, it is time to compile the all the results and provide them to the user. The Groundtruth Compilation component periodically checks each active job in the job submission table to determine if all its tasks have been purged. If so, this function compiles all the aggregated results corresponding to this job into a JSON file, stores this at a user-specified location and notifies the user.

% \iffalse
% \begin{figure}[h]
%   \centering
% \begin{minipage}{3.0in}
%   \includegraphics[width=3.0in]{figs/Overview/State-Transitions}
%   \vspace*{-0.15in}
%  \caption{State transitions of \sysname's jobs,tasks and HITs}
% \label{fig:State-Transitions}
% \end{minipage}
% \end{figure}
% \fi

% \subsection{Extensibility, Evolvability and Scalability of \sysname}

% ML for machine vision is a rapidly evolving field and new web-UIs might be needed in the future to produce new kinds of groundtruth data. The design of \sysname makes it easy to add new templates in a modular manner without changing most of the core components. For a new template, a developer need only add a specific result aggregator, result evaluator and web-UI for each new template. 

% \satyam's architecture is evolvable; each component (\eg Web-UIs, Quality Control Algorithms ({\it groundtruth-fusion}), HIT management functions) can be independently modified as long as it conforms to well defined interfaces. We expect future research to improve upon our current algorithms along various dimensions such as accuracy, speed of execution \etc

% The current architecture allows each \sysname component to be deployed as separate cloud functions (e.g. Azure functions). Further, every single component is highly parallelizable. For example, Task Generator can be heavily parallelized with one thread for each image/video clip. Similarly, Results Aggregator is also highly parallelizable with one thread for each \sysname-task. 
% }\fi

\iffalse
As described in Section~\ref{sec:gt} there are 
We have designed \sysname with three main goals. 
\begin{itemize}
    \item Templates – description and examples of where they are used
    \item Template to Tasks
    \item Amazon HIT Launching logic
    \item Fusion, Consensus Algorithms and Relaunching
    \item Accept Reject Criterion and Paying
    \item Results saving
\end{itemize}
%\usepackage{}
Various components
\begin{itemize}
    \item Templates – description and examples of where they are used
    \item Template to Tasks
    \item Amazon HIT Launching logic
    \item Fusion, Consensus Algorithms and Relaunching
    \item Accept Reject Criterion and Paying
    \item Results saving
\end{itemize}
\fi

==> Satyam ArXiv/pricing.tex <==
\section{HIT management}
\label{sec:payments}

These components manage the interactions between \sysname and AMT such as launching HITs for the tasks, estimating and adapting the price of HITs to match user specifications, filtering under-performing workers, submitting results to the quality control component, and finally, making/rejecting payments for tasks that have completed. 

\parab{HIT Generator}
This component creates HITs in AMT using the web-service API that AMT provides~\cite{mturk_sdk} and associates these HITs with an entry in the {\it HIT-Table} (which also contains pricing metadata, as well as job/task identification). It ensures that every unfinished task in the \satyam-task table has at least one HIT associated with it in AMT. It does this by comparing the number of unfinished tasks in the Task-Table for each GUID and price level against the number of unfinished HITs in the HIT-Table and determines the deficit. Because a single HIT may comprise multiple tasks, \sysname computes the number of extra HITs needed to fill any deficit and launches them. To determine which HITs have been worked on, as soon as a worker submits a HIT, \satyam records this in the HIT-Table.

\parab{HIT Price Adaptation}
Several organizational and state laws require hourly minimum wage payments. Moreover, hourly wages are easier for users to specify. However, payments in AMT are disbursed at the granularity of a HIT. Thus, \satyam must be able to estimate the ``reasonable'' time taken to do a HIT and translate it to price per HIT based on the desired hourly rate. The time taken for a HIT can vary from a few seconds to several minutes and depends on three factors: (a) the type of the template (\eg segmentation tasks take much longer than classification tasks); (b) even within the same template, more complex jobs can take longer \eg scenes with more cars at a busy intersection; (c) finally, different workers work at different rates. 

To estimate HIT completion times, \satyam instruments the web-UIs provided to workers and measures the time taken by the worker on the HIT. As each job progresses, \satyam continuously estimates the median time to HIT completion per job (considering only approved HITs). It uses this value to adjust the price for each future HIT in this particular job. Using this, \satyam's price per HIT converges to conform to hourly minimum wage payments (\secref{sec:eval}).

% \iffalse{
% Given that different annotation tasks take different time, \satyam must estimate
% \satyam allows users to specify an hourly rate that they wish to pay to the AMT workers.    
% A key question often that is hard to answer for \sysname users is what should be the price of a HIT? This question is governed by two factors. First, AMT is an open market and workers like to choose HITs that pay them the most in the shortest amount of time and those that are interest them. Thus, a HIT with a price too low will remain undone. Second, while a \sysname user might want to pay as low as possible, ethics and minimum pay standards employed by companies impose constraints on the minimum hourly rates that must be paid to workers. 

% %As prior work has pointed out, there is clearly a correlation between time to complete a HIT and price~\cite{xxx}.
% Unfortunately, the time to complete a job depends on at least two factors. First, it depends on the job category (\figref{fig:timeCDF}): task completion times are high for more visually complex tasks like counting, detection and classification, and they also vary a lot. Within the same job category, time to complete tasks can depend on the data (\figref{fig:timeCDF_counting}): KITTI has around 10 vehicles on average, and CARPK around 45 in each image, and the distribution of worker task completion times varies significantly across these datasets. (As an aside, both these figures have a long tail: we have seen several cases where workers start tasks but sometimes finish it hours later).

% Given this, we believe \satyam should support \textit{adaptive pricing}: users can specify a price range within which \satyam can adaptively adjust prices based on worker task completion rates. Such a strategy would adapt both to task complexity and visual complexity in the data. \looseness=-1
% }\fi

\parab{\sysname HIT Payments} 
Once a task is aggregated, deserving workers must be paid. \satyam relies on the fusion algorithms to determine whether a result should be \textit{accept}-ed or not (\secref{sec:fusion}). A single HIT may include multiple \satyam-tasks; \satyam's HIT Payments component computes the fraction of \textit{accepted} results in a HIT across all of these tasks and pays the worker if this fraction is above a threshold.

\parab{Worker Filtering}
Worker performance can vary across templates (\eg good at classification but not segmentation), and across jobs within a given template (\eg good for less complex scenes but not for more complex ones). To minimize rejected payments, \satyam tracks worker performance and avoids recruiting them for tasks they might perform poorly at. To do this, as \satyam rejects payments to undeserving workers for a certain task, it tracks worker approval rates (using the AMT-supplied opaque workerID) for each job and does not serve HITs to workers that have low approval rates (lower than 50\% in our implementation). While serving HITs to workers with past high performance history allows \satyam to be efficient, \satyam must also explore and be able to discover new workers. Thus, \satyam allows workers with good approval rates to work on 80\% of the HITs, reserving the rest for workers for whom it does not have any history. As shown in our evaluations~\ref{sec:evaluation:workerFiltering}, worker filtering results in much fewer overall rejections. 

% Certain workers might perform well for easy templates (\eg classification) but might not do so for more complex templates (\eg segmentation). Worker performance may also vary across different jobs for the same template depending on the number and difficulty of the annotations (\eg scenes with a large number of objects to draw boxes around versus scenes with less objects). 


%We shall now outline how the deviation is measured for each template.

\parab{\sysname Task Purge}
This component, triggered whenever a result is aggregated, removes completed tasks from the Task Table so that they no longer show up in any future HITs.

% Whenever a result is aggregated, this component is triggered. It reads the {\it Aggregated-Results-Table} and removes all the completed \sysname-tasks from the Task-Table. 



% \iffalse
% {
% \parab{Image/Video Classification} For these templates, we approve the HITs and pay all the workers whose selected category matches that of the aggregated result. As discussed in Section~\ref{sec:fusion:classification}, sometimes there is no clear wining category, i.e. no category achieves a super-majority. In these cases, we first rank the categories in descending order of the number of worker who selected them. Then we choose the minimum number of categories such that the combined number of workers that selected them exceeds super-majority and approve all their HITs and pay them.

% \parab{Counting in Images/Videos}
% For these templates, we simply consider workers with counting error fraction less than  $\epsilon$ (Section~\ref{sec:fusion:counting}) from the aggregated count as the deserving workers that need to be paid.

% \parab{Multi-object Localization and Tracking }
% We consider deserving workers as those whose work has contributed to most of the objects in the image/video. Thus, for each worker we count the number of objects a certain worker's bounding boxes contributed to. If this number is greater than a certain fraction (50\% in our implementation) more than the total number of objects in the image/object we consider the worker as deserving and approve (pay) their work.
% }
% \fi

==> Satyam ArXiv/refs.tex <==
\bibliography{references.bib}
\bibliographystyle{plainnat}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> Satyam ArXiv/related.tex <==
\section{Related Work}
\label{sec:related}

\parab{Image recognition using crowdtasking}
ImageNet training data for classification was generated using AMT, and uses majority voting for consensus~\cite{ImageNet}. Prior work~\cite{bbox_crowd12} has also shown crowdtasking to be successful for detection: unlike \sysname, in this work, quality control is achieved by using workers to rate other workers, and majority voting picks the best bounding box. These use one-off systems to automate HIT management and consensus, but do not consider payment management. \sysname achieves comparable performance to these systems but supports more vision tasks. Third party commercial crowdtasking systems exist to collect groundtruth for machine vision~\cite{crowdflower,spare5_website}. Other approaches have developed one-off systems built on top of AMT for more complex vision tasks, including feature generation for sub-class labeling~\cite{Deng13}, and sentence-level textual descriptions~\cite{VisualGenome,Datasift14}: more generally, future machine vision systems will need annotated groundtruth for other complex annotations including scene characterization, activity recognition, visual story-telling~\cite{CSsurvey} and we have left it to future work to extend \sysname to support these. \looseness=-1

\parab{Crowdtasking cost, quality, and latency} Prior work has extensively used multiple worker annotations and majority voting to improve quality~\cite{ImageNet,bbox_crowd12}. For binary classification tasks in a one-shot setting, lower cost solutions exist to achieve high quality~\cite{Karger11} or low latency~\cite{KrishnaError}. For top-$k$ classification (e.g., finding the $k$ least blurred images in a set) several algorithms can be used for improving crowdtasking consensus~\cite{Topk16}. Other work has explored this cost-quality tradeoff~\cite{Challenges16} in different crowd-tasking settings: de-aliasing entity descriptions~\cite{Waldo17,Khan16}, or determining answers to a set of questions~\cite{CrowdDQS17}. \sysname devises novel automated consensus algorithms for image recognition tasks based on the degree of pixel overlap between answers.

\parab{Crowdtasking platforms} Many marketplaces put workers in touch with requesters for freelance work~\cite{Guru,Freelancer,99design}, for coders~\cite{TopCoder}, for software testing~\cite{Mob4Hire,utest}, or for generic problem solving~\cite{Innocentive}. \satyam adds automation on top of an existing generic marketplace, AMT. Other systems add similar kinds of automation, but for different purposes. Turkit~\cite{turkit} and Medusa~\cite{Medusa} provide an imperative high-level programming language for human-in-the-loop computations and sensing respectively. Collaborative crowdsourcing~\cite{collabcrowd} automates the decomposition of more complex tasks into simpler ones, and manages their execution. 

% \satyam is complementary: by focusing on vision tasks, it can provider a higher level of abstraction and automate result aggregation.

% \parab{Deep Neural Networks} \satyam is motivated by the development of deep neural nets that require significant amounts of annotated groundtruth for training and testing. It also leverages techniques for retraining these networks.

==> appendices.tex <==
\newpage
\appendix
\renewcommand\thefigure{A.\arabic{figure}}
\setcounter{figure}{0}

%% Datasets
%% Sensitivity
%% Portal
%% Samples
%% Examples
%% Error Analysis

\section{Appendix}
%\section{Illustrations}

% Things that should go in here:
% \begin{itemize}[topsep=1pt,itemsep=0pt,leftmargin=*]
%     \item Pseudo code for tricky algorithms
%     \item Screen shots of templates
%     \item Screen shot of worker view
%     \item Sample images for some of the tasks (tracking, localization \etc)
%     \item project webpage of aggregated results, yolo coco and satyam retrain comparison...
%     \item $\ldots$
% \end{itemize}

\begin{figure*}[t]
\centering
  \begin{minipage}{0.66\columnwidth}
  \centering
  \includegraphics[width=0.95\columnwidth]{figs/MotivationAndAMTOverview/DetectionResult_lowres.pdf}
  %\vspace*{-0.15in}
  \caption{Example Results of \satyam Detection from KITTI}
  \label{fig:DetResult}
 \end{minipage}
\begin{minipage}{0.66\columnwidth}
  \centering \includegraphics[width=0.95\columnwidth]{figs/MotivationAndAMTOverview/SegResult_lowres.pdf}
  %\vspace*{-0.15in}
  \caption{Example Results of \satyam Segmentation from PASCAL}
  \label{fig:SegResult}
\end{minipage}
\begin{minipage}{0.66\columnwidth}
 \centering\includegraphics[width=0.95\columnwidth]{figs/MotivationAndAMTOverview/TrackingResult_lowres.pdf}
  %\vspace*{-0.15in}
  \caption{Example Results of \satyam Tracking from KITTI}
  \label{fig:TrackingResult}
\end{minipage}
\end{figure*}

\subsection{ML Benchmark Datasets Used in Evaluation}
\label{sec:eval:datasets}
 
\parab{Image Classification (ImageNet-10)} We create this dataset by picking all the images corresponding to 10 classes commonly seen in video surveillance cameras from the ImageNet~\cite{ImageNet} dataset. Our dataset contains 12,482 images covering these classes: cat, dog, bicycle, lorry-truck, motorcycle, SUV, van, female person and male person.  

\parab{Video Classification (JHMDB-10)} For this data set we pick all the video clips from the JHMDB~\cite{JHMDB} data set corresponding to to 10 common human activities: clap, jump, pick, push, run, sit, stand, throw, walk and, wave (a total of 411 video clips).

\parab{Counting in Images (CAPRK-1)} We create this data set by selecting 164 drone images taken from one parking lot from CAPRK~\cite{carpk} (a total of 3,616 cars).

\parab{Object Detection in Images (KITTI-Object)}
We create this data set by considering 3 out of 8 classes (cars, pedestrians and cyclists) in the KITTI~\cite{KITTI}  data set with 8000 images (a total of 20,174 objects.). The groundtruth in KITTI established using LiDAR mounted on the car. 

\parab{Object Segmentation in Images (PASCAL-VOC-Seg)} %PASCAL-VOC \cite{pascalvoc} is a standardized image dataset for object classification, detection, segmentation, action classification, and person layout. 
We create this data set by choosing XXX images from the PASCAL-VOC \cite{pascalvoc} data set that have segmentation labels, including the groundtruth of both class- and instance-level segmentation, corresponding to a total of XXX objects of 20 different classes.

\parab{Tracking in Videos (KITTI-Trac)} For this dataset we chose all 21 video clips that were collected from a moving car from KITTI~\cite{KITTI} (about 8000 frames), but evaluate tracks only for 2 classes -- cars and pedestrians. During the pre-processing step, these 21 video clips were broken into 276 chunks of length 3 seconds each with a 0.5 second overlap between consecutive chunks.

\parab{Traffic Surveillance Video Stream Data (SURV)} We extracted images at 1~frame/minute from the video streams of 4 live HD quality traffic surveillance cameras, over one week (7 days) between 7:00~am and 7:00~pm each day. These cameras are located at major intersections in two U.S cities. We label the dataset corresponding to each of the four cameras as SURV-1, SURV-2, SURV-3 and SURV-4 respectively. 



\subsection{Samples of Groudtruth Images/Video Obtained by \satyam}
\label{sec:samples}
Figures~\ref{fig:DetResult},~\ref{fig:SegResult} and~\ref{fig:TrackingResult} show some examples of groundtruth obtained using \satyam for detection, segmentation and tracking templates respectively.



\subsection{Examples of \satyam tasks seen by workers}
\label{sec:portal}
The \satyam portal can be visited at ~\cite{satyamportal_website}. Here we provide a few example screenshots of the task pages that AMT workers see for each template in Figures~\ref{fig:imClassfication_taskpage},~\ref{fig:counting_taskpage},~\ref{fig:imDetection_taskpage},~\ref{fig:imSegmentation_taskpage}, and ~\ref{fig:tracking_taskpage}. Figure~\ref{fig:mturk} depicts a typical view of an AMT worker, when they choose among the many HITs available to them.



\begin{figure}[h]
  \centering
  \includegraphics[width=\columnwidth]{figs/appendix/ImageClassification.PNG}
  %\vspace*{-0.15in}
  \caption{Image Classification Task Page}
  \label{fig:imClassfication_taskpage}
\end{figure} 

\begin{figure}[h]
  \centering
  \includegraphics[width=\columnwidth]{figs/appendix/Counting.PNG}
  %\vspace*{-0.15in}
  \caption{Object Counting Task Page}
  \label{fig:counting_taskpage}
\end{figure}

\begin{figure}[h]
  \centering
  \includegraphics[width=\columnwidth]{figs/appendix/ImageDetection.PNG}
  %\vspace*{-0.15in}
  \caption{Object Detection and Localization Task Page}
  \label{fig:imDetection_taskpage}
\end{figure}

\begin{figure}[h]
  \centering
  \includegraphics[width=\columnwidth]{figs/appendix/Segmentation.PNG}
  %\vspace*{-0.15in}
  \caption{Object Segmentation Task Page}
  \label{fig:imSegmentation_taskpage}
\end{figure}

\begin{figure}
  \centering
  \includegraphics[width=\columnwidth]{figs/appendix/Tracking.pdf}
  %\vspace*{-0.15in}
  \caption{Multi-Object Tracking Task Page}
  \label{fig:tracking_taskpage}
\end{figure}

\begin{figure}[h]
  \centering
  \includegraphics[width=\columnwidth]{figs/appendix/mturk.PNG}
  %\vspace*{-0.15in}
  \caption{Amazon MTurk HITs Web Portal}
  \label{fig:mturk}
\end{figure} 

\subsection{Examples of Mismatches between \satyam and Benchmarks}
\label{sec:mismatches}

In this section we provide some interesting examples of mismatch between groundtruth in the benchmark data sets and that obtained by \satyam to provide insights to the reader. 

Figure~\ref{fig:vantruck1} shows errors in the classification template due to linguistic confusion where, while in ImageNet these vehicles were labeled as vans, \satyam yielded the class label as trucks.
Figure~\ref{fig:segmentation_error} shows an error by the human annotator in the benchmark dataset for the segmentation template where the human misses marking the  truck in the scene whereas these are marked in the groundtruth obtained from \satyam.
Figure~\ref{fig:count_error} is an example of the confusion that human annotators experience when counting in groundtruth data sets where there are partially visible cars which are open to interpretation of the annotator as to whether it should be included in the count.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.45\columnwidth]{figs/appendix/van_truck1.jpg}
    \includegraphics[width=0.45\columnwidth]{figs/appendix/van_truck2.jpg}
    \caption{Linguistic confusion between van and truck}
    \label{fig:vantruck1}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.32\columnwidth]{figs/appendix/2007_000364.jpg}
    \includegraphics[width=0.32\columnwidth]{figs/appendix/2007_000364.png}
    \includegraphics[width=0.32\columnwidth]{figs/appendix/2007_000364_aggregated.PNG}
    \caption{Example of missing segmentation labels from PASCAL. From left to right: raw image, PASCAL label, \satyam label. \satyam segments a small truck on the top left corner which was not present in the ground truth.}
    \label{fig:segmentation_error}
\end{figure}


% \begin{figure}[h]
%     \centering
%     \includegraphics{figs/appendix/van_truck2.jpg}
%     \caption{Another example of linguistic confusion between van and truck}
%     \label{fig:vantruck2}
% \end{figure}


\subsection{Tracking Error Analysis}
\label{sec:error}

To understand tracking errors, we explored worker performance at different positions in the chunk (\figref{fig:tracking_error_chunk}): we found that, as workers get to the end of a chunk, they tend not to start tracking new objects. Decreasing the chunk size and increasing the overlap among consecutive chunks would increase accuracy, at higher cost. 

% We have left an understanding of this to future work, in part because \satyam's groundtruth is of high-enough quality that models re-trained with \satyam perform identically with benchmark-retrained models, as we discuss next.

% A detailed analysis of errors in the tracking template indicated that a large part of the this loss in accuracy comes from the fact that workers tend to not start new tracks towards the end of the video chunk. Consequently, we believe that decreasing the chunk size and increasing the overlap among consecutive chunks will increase the accuracy, however, this comes at a higher cost, as the more workers are needed to annotate the larger number of video chunks. 

\begin{figure}
    \centering
     \includegraphics[width=\columnwidth]{figs/eval/video_confusionMat.pdf}
%   %\vspace*{-0.15in}
 \caption{Confusion Matrix of \satyam Result on JHMDB}
 \label{fig:confMatVideo}
\end{figure}


\begin{figure}[h]
    \centering
    \includegraphics[width=\columnwidth]{figs/appendix/count_error.pdf}
    \caption{Example of counting error resulting from partially visible cars}
    \label{fig:count_error}
\end{figure}

\begin{figure}
  \centering
  \includegraphics[width=\columnwidth]{figs/eval/TrackingErrorDistribution.eps}
  %\vspace*{-0.15in}
  \caption{Tracking Error Distribution over 30 Frame Video Chunk}
  \label{fig:tracking_error_chunk}
\end{figure}

\subsection{Parameter Sensitivity}
\label{sec:evaluation:paramChoices}

\satyam's groundtruth fusion and result evaluation algorithms have several parameters and \figref{fig:accuracy} presents results for the best parameter choice. We have analyzed the entire space of parameters to determine the parameters that \satyam performance most crucially depends upon in terms of accuracy, latency and cost.

Image classification is sensitive only to two parameters: $n_{min}$, the minimum number of results before aggregation can commence, and $\beta$, the fraction determining the super-majority. The upper graph in \figref{fig:param:image_classification} shows how classification accuracy varies as a function of these two parameters. Because the cost and latency of groundtruth collection varies with parameters, the lower graph shows the cost (blue bars) and the latency (red bars) for each parameter choice. From this, we can see that when $n_{min}\ge 3$  and $\beta \ge 0.7$ the accuracy does not improve significantly, however, cost and latency increase. This indicates that $n_{min}=3$ and $\beta = 0.7$ are good parameter choices, with high accuracy, while having moderate cost and latency. \looseness=-1

We have conducted similar analyses for video classification (\figref{fig:param:video_classification}), counting (\figref{fig:param:counting}), object detection (\figref{fig:param:localization}), and tracking (\figref{fig:param:tracking}). Space constraints preclude a detailed discussion, but the key conclusions are:
(a) All job categories are sensitive to $n_{min}$, the minimum number of results before \satyam attempts to aggregate results;
(b) Each category is sensitive to one other parameter. For classification, this is the $\beta$ parameter that determines the super-majority criterion. For counting, it is the error tolerance $\epsilon$. For detection and tracking, it is $\eta_{cov}$, the fraction of corroborated groundtruth elements; and
(c) In each case, there exists a parameter settings at which provides good groundtruth performance at moderate cost and latency.

\begin{figure}
  \centering
%   \includegraphics[width=2.8in]{figs/eval/ParamSweep_ImageClassification.eps}
  \includegraphics[width=0.95\columnwidth]{figs/eval/ParamSweep_ImageClassification_LargerFont.eps}
  %\vspace*{-0.15in}
  \caption{Accuracy, Latency and Cost: Image Classification}
  \label{fig:param:image_classification}
\end{figure}

\begin{figure}
  \centering
  \includegraphics[width=\columnwidth]{figs/eval/ParamSweep_VideoClassification.eps}
  %\vspace*{-0.15in}
  \caption{Accuracy, Latency and Cost: Video Classification}
  \label{fig:param:video_classification}
\end{figure}

\begin{figure}
  \centering
  \includegraphics[width=\columnwidth]{figs/eval/ParamSweep_Counting.eps}
  %\vspace*{-0.15in}
  \caption{Accuracy, Latency and Cost: Counting}
  \label{fig:param:counting}
\end{figure}

\begin{figure}
  \centering
  \includegraphics[width=\columnwidth]{figs/eval/ParamSweep_Detection.eps}
  %\vspace*{-0.15in}
  \caption{Accuracy, Latency and Cost: Detection}
  \label{fig:param:localization}
\end{figure}

\begin{figure}
  \centering
  \includegraphics[width=\columnwidth]{figs/eval/ParamSweep_Tracking.eps}
  %\vspace*{-0.15in}
  \caption{Accuracy, Latency and Cost: Tracking}
  \label{fig:param:tracking}
\end{figure}



%  \begin{figure}
%   \centering
%      \includegraphics[width=\columnwidth]{figs/eval/ApprovalTimeSeries.eps}
%   %\vspace*{-0.15in}
%   \caption{Tracking Approval rates through Worker Filtering}
%   \label{fig:trackingApprovalRate}
%  \end{figure}

% \begin{figure}
%   \centering
%   \includegraphics[width=\columnwidth]{figs/eval/ApprovalTimeSeries.eps}
%   %\vspace*{-0.15in}
%   \caption{Approval Rates of Tracking Task}
%   \label{fig:trackingApprovalRate}
% \end{figure}


==> emulations.tex <==



\section{Lessons and Future Work}
\label{sec:learnings}

We have had significant experience with \satyam, having launched over 162,000 HITs and 470,000 \satyam-tasks to nearly 10,000 workers in the past year or so. We now we describe lessons learned from our use of \satyam, and discuss ways to improve \satyam's efficiency and usability.

\iffalse
{
\begin{table}[h]
\centering
\footnotesize
\begin{tabular}{|l|l|l|}\hline
{\bf Web-UI Template} & {\bf Original} & {After Filtering} \\ \hline\hline
Image Classification & 89\% & 90.3\% \\ \hline
Video Classification & 88.7\% & 91.4\% \\ \hline
Localization in Images & 75\% & 82.9\% \\ \hline
Tracking in Videos & 68.1\% & 86.6\% \\ \hline
Counting in Images & 92.4\% & 94\% \\ \hline
\end{tabular}
\caption{Approval Rates for various \sysname templates}
\label{tab:approvals}
%\vspace{-0.1in}
\end{table}
}\fi
% \begin{figure}
%   \centering
%   \includegraphics[width=\columnwidth]{figs/eval/ApprovalCanary.eps}
%   %\vspace*{-0.15in}
%   \caption{Approval Rates with Worker Filtering}
%   \label{fig:workerFilter}
% \end{figure}

% \begin{figure}
%   \centering
%   \includegraphics[width=\columnwidth]{figs/eval/ApprovalTimeSeries.eps}
%   %\vspace*{-0.15in}
%   \caption{Approval Rates of Tracking Task}
%   \label{fig:trackingApprovalRate}
% \end{figure}

% \subsection{Worker Filtering}
% \label{sec:learnings:workerFiltering}


% As seen from Table~\ref{tab:approvals}, while the classification tasks have a high approval rate of over 90\%, localization and tracking tasks have a lower approval rates of 70\% and 60\% respectively. This indicates for more complex tasks, fewer fraction of untrained workers in the AMT system, perform satisfactorily. High worker rejection rates for complex tasks not only adversely effects \sysname by wasting computing resources but also wastes workers' moral as they feel they wasted their precious time. Thus, it is useful to be able to preferentially provide HITs corresponding to a job to workers who have historically performed well on that job. In order to test our hypothesis, we designed and emulated a worker filtering mechanism on data obtained from our evaluation of \sysname.

% allowing 80\% of HITs are preferentially provided to good workers while 20\% of the HITs are provided to new workers for whic
% Our mechanism must preferentially provide HITs to historically well performing workers while also exploring new workers for potential new performers. For each job, we maintain and update the approval rate for each worker as the results for the job are aggregated. Workers with approval rates higher than 50\% are deemed ``good workers'' and 80\% of the HITs are preferentially provided to these  good workers while 20\% of the HITs are provided to new workers who have not been evaluated. 

\parae{Evaluation} Table~\ref{tab:approvals} shows this simple mechanism significantly improves the approval rate of the workers for the complex templates: object detection and tracking approval rates increase by 7\% and 22\% respectively. Moreover, this mechanism works well throughout the duration of the job: with worker filtering, approval rates start high and remain higher than without approval (\figref{fig:trackingApprovalRate}).

% such as tracking from 60\% to 20\%. Figure~\ref{fig:xxx} shows how the approval rate for a tracking template job changes over time with and without filtering. As seen from Figure~\ref{fig:xxx}, worker filtering keeps the approvals consistently at a high rate and thus engaging workers who perform well. We hope to improve upon these initial algorithms for worker filtering and incorporating it into the \sysname system.

% \subsection{Adaptive Pricing}
% \label{sec:learnings:adaptivePricing}

\parab{Adaptive Pricing}
A key question often that is hard to answer for \sysname users is what should be the price of a HIT? This question is governed by two factors. First, AMT is an open market and workers like to choose HITs that pay them the most in the shortest amount of time and those that are interest them. Thus, a HIT with a price too low will remain undone. Second, while a \sysname user might want to pay as low as possible, ethics and minimum pay standards employed by companies impose constraints on the minimum hourly rates that must be paid to workers. 

%As prior work has pointed out, there is clearly a correlation between time to complete a HIT and price~\cite{xxx}.
Unfortunately, the time to complete a job depends on at least two factors. First, it depends on the job category (\figref{fig:timeCDF}): task completion times are high for more visually complex tasks like counting, detection and classification, and they also vary a lot. Within the same job category, time to complete tasks can depend on the data (\figref{fig:timeCDF_counting}): KITTI has around 10 vehicles on average, and CARPK around 45 in each image, and the distribution of worker task completion times varies significantly across these datasets. (As an aside, both these figures have a long tail: we have seen several cases where workers start tasks but sometimes finish it hours later).

Given this, we believe \satyam should support \textit{adaptive pricing}: users can specify a price range within which \satyam can adaptively adjust prices based on worker task completion rates. Such a strategy would adapt both to task complexity and visual complexity in the data. \looseness=-1

% \sysname already maintains statistics regarding how long workers take for each HIT, recording the time difference between the time the worker was served the HIT to the time it was submitted. Figure~\ref{fig:timeCDF} depicts the CDF of times taken to perform a task for each of the five templates. Task completion times depend on the complexity of the task and exhibit large variability (the x-axis is in log-scale). One strategy is to use the median value of task completion times for each job and use that for determining the price per HIT. For example, it can be used to ensure the minimum payrate constraints for each job. Further, adaptive exploration schemes can be developed that try various price points.


% \begin{figure}
%   \centering
%   \includegraphics[width=\columnwidth]{figs/eval/timePerResult.eps}
%   %\vspace*{-0.15in}
%   \caption{CDF of Time Spent Per Task of All Job Categories}
%   \label{fig:timeCDF}
% \end{figure}

% \begin{figure}
%   \centering
%   \includegraphics[width=\columnwidth]{figs/eval/countingTimePerResult.eps}
%   %\vspace*{-0.15in}
%   \caption{CDF of Time Per Counting Task over Different Datasets}
%   \label{fig:timeCDF_counting}
% \end{figure}

% \subsection{Managing Cognitive Complexity}
% \label{sec:learning:cognitivecomplexity}

\parab{Managing Cognitive Complexity}
Although we have tested \satyam on images with significant visual complexity (\eg 20-30 cars) and workers seem to perform well, \satyam will need mechanisms to adapt to visual complexity to avoid cognitive overload. It already uses a simple, non-adaptive strategy: chunking video clips into fixed length segments to manage cognitive overload. We arrived at this strategy by experimenting with longer videos and finding that no worker completed these tasks. \satyam could adaptively determine, based on HIT uptake, whether a particular job has high cognitive load, then, adapt chunk sizes dynamically for video, or tesselate images. \looseness=-1

\parab{A Unifying Mechanism: The Canary}
The adaptive capabilities described above require estimates for worker approval rates and task completion times. These depend not just on the job category, but also on the complexity of the data itself. We are currently experimenting with a \textit{canarying} mechanism, whereby \satyam sends a small fraction of the user-submitted data to workers to learn these parameters, then uses these when obtaining groundtruth for the complete set.





==> ground_truth.tex <==
\begin{figure*}[h]
  \centering
  \begin{minipage}{2.1in}
\includegraphics[width=1.9in]{figs/MotivationAndAMTOverview/MotivationBeforeAfterFineTuning}
  \vspace*{-0.15in}
 \caption{Improvement of performance with fine tuning}
\label{fig:MotivationYoLoPerformance}
\end{minipage}
\begin{minipage}{2.1in}
  \includegraphics[width=1.9in]{figs/MotivationAndAMTOverview/MotivationExampleYoLoBefore}
  \vspace*{-0.15in}
 \caption{Example of YoLo's output before fine-tuning (from data set $Cam1$) }
\label{fig:MotivationYoLoBefore}
\end{minipage}
\begin{minipage}{2.1in}
\includegraphics[width=1.9in]{figs/MotivationAndAMTOverview/MotivationExampleYoLoAfter}
  \vspace*{-0.15in}
 \caption{Example of YoLo's output after fine-tuning (from data set $Cam1$)}
\label{fig:MotivationYoLoAfter}
\end{minipage}
\end{figure*}

\section{Obtaining Groundtruth using AMT}
\label{sec:gt}

In this section we first motivate the need for using crowdtasking systems such as AMT for machine vision based systems and then explain the various challenges involved in obtaining groundtruth. To guide us we we use a practical traffic video surveillance system as an example. 

\subsection{Need for Groundtruth}
\label{sec:gt:NeedForFineTuning}
The performance of ML systems is only as good as the data they are trained on.
There are several publicly available pre-trained ML models for various machine vision scenarios that are trained on benchmark data sets. However, directly employing these ML models in the field often results in poor accuracy, since the nature and conditions of the images in the field are often very different from those in the benchmark data sets. A common approach is to start with a publicly available ML model, but then follow it up with a fine-tuning step where the model is trained further on actual data from the field. In many practical deployments, testing and fine-tuning becomes a periodic activity to keep adapting to changing conditions and to maintain performance guarantees.

In order to provide the reader with an intuition we leverage a real life example -- a vision system that locates cars in traffic video surveillance images. We obtain HD quality images from four busy traffic intersections in two  prominent U.S. cities. Images are collected between 7:00 A.M to 7:00 P.M over a week (7 days) at one minute intervals to cover all the different conditions in the scene -- a total of 5000 images/camera (20000 images). We use a popular deep neural network, YOLO~\cite{yolo}, that generates bounding boxes for objects of interest (cars). We obtain groundtruth bounding boxes for the cars in each images using \satyam. The data for each camera is partitioned into 20\% testing and 80\% training data sets. 

We start with a publicly available pretrained ML model YoLo-Coco -- YoLo trained on the CoCo data set~\cite{XXX}. We also then fine-tune YoLo-CoCo  specifically each camera, by retraining its last-layer (a common practice) using the training data for that camera. As depicted in Figure~\ref{fig:MotivationYoLoPerformance},  YoLo-CoCo performs poorly on all the four cameras with a precision of under 50\%. This poor performance occurs because the characteristics of the specific camera footage e.g. angle, background scenery etc are often very different from that in the training images in the CoCo dataset. After fine-tuning, (YoLo-FineTuned), there is a dramatic improvement in accuracy (> 80\%) for each camera. Figures~\ref{fig:MotivationYoLoBefore} and~\ref{fig:MotivationYoLoAfter} show an example of YoLo output before and after the fine-tuning. 


\subsection{Labling Effort}
\label{sec:gt:effort}
In order to fine tune YoLo, the groundtruth required for each image is the set of all bounding boxes for each car (specified by the pixel coordinates of their top left and right bottom corners). With about 15-25 cars per image, the process of drawing a box around each object takes on average 90 seconds per image and amounts to approximately 125 man-hours per camera. This example demonstrates how even this relatively ``small scale'' experiment requires a huge manual effort in terms of groundtruth annotation.

\subsection{AMT Overview and Terminology}
\label{sec:gt:Need}
AMT provides on-demand access to a pool of workers that can potentially help with the groundtruth annotation effort. However, one has very little/no direct control over these workers and they are free to choose among the several thousands of jobs in the AMT platform based on their preferences. 

\parab{Human Intelligence Task (HIT)} HIT is the minimum unit of work for which a worker is paid for upon finishing it "acceptably". HITs appear as a webpages to the worker and are typically tasks that can be done within the confines of a browser. In our example, one HIT would comprise a worker drawing boxes around all the cars in a single image. 

\parab{Requesters} are users who create HITs and are responsible for accepting (paying) or rejecting (not paying) the work performed by the workers.

\subsection{Challenges in Using AMT}
\label{sec:gt:challenges}

In this section we describe the various steps and challenges involved in using AMT for groundtruth collection.

\parab{Creating Web-UI HITs}
The first step to using AMT is to creating a web application that displays a specific image/video clip equipped with a UI and appropriate instructions that makes it easy for untrained workers to annotate groundtruth easily and accurately. Design of these UIs can be extremely challenging and there exists a large body of research that focuses on UI design for various tasks e.g.~\cite{VATIC}. Often the expertise and effort needed to develop a web-UI is a deterrent to using crowdtasking platforms. 
 
\parab{Quality Control} 
Workers in AMT are untrained and may not generate a good annotation. In our traffic surveillance example, workers may miss drawing boxes around cars either due to negligence, inexperience with the UI or simply lack of interest. In our experience, a significant fraction of the results from the workers are always incorrect, especially for more sophisticated machine vision applications. Thus, the onus of determining which results are acceptable solely lies on the requesters, who have to typically inspect the results manually. For incorrect results, these annotation tasks may have to be resent to more workers. For large data sets this manual intervention, quickly becomes unscalable. 

\parab{HIT Management -- Launching and Payments} 
A HIT is typically launched for each image and launching tens of thousands of HIT annotations requires automation using AMT web service APIs. Further, when some annotations are unacceptable, these must be identified and re-launched to more workers. The requester is also responsible identifying and paying the deserving workers while rejecting the rest. This is once again a manual process and does not scale. 



==> implementation.tex <==
\section{Implementation on Azure}
\label{sec:impl}
\sysname has been implemented on Azure and written primarily using C#, javascript and the ASP .Net framework comprising a total of XXX lines of code. As described


Various components
\begin{itemize}
    \item Templates – description and examples of where they are used
    \item Template to Tasks
    \item Amazon HIT Launching logic
    \item Fusion, Consensus Algorithms and Relaunching
    \item Accept Reject Criterion and Paying
    \item Results saving
\end{itemize}

==> refs.tex <==
\bibliography{references.bib}
\bibliographystyle{plainnat}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:

